Post-Quantum Simulatable Extraction with Minimal Assumptions: Black-Box and Constant-Round

From the minimal assumption of post-quantum semi-honest oblivious transfers, we build the first $\epsilon$-simulatable two-party computation (2PC) against quantum polynomial-time (QPT) adversaries that is both constant-round and black-box (for both the construction and security reduction). A recent work by Chia, Chung, Liu, and Yamakawa (FOCS'21) shows that post-quantum 2PC with standard simulation-based security is impossible in constant rounds, unless either $\mathbf{NP} \subseteq \mathbf{BQP}$ or relying on non-black-box simulation. The $\epsilon$-simulatability we target is a relaxation of the standard simulation-based security that allows for an arbitrarily small noticeable simulation error $\epsilon$. Moreover, when quantum communication is allowed, we can further weaken the assumption to post-quantum secure one-way functions (PQ-OWFs), while maintaining the constant-round and black-box property. Our techniques also yield the following set of constant-round and black-box two-party protocols secure against QPT adversaries, only assuming black-box access to PQ-OWFs: - extractable commitments for which the extractor is also an $\epsilon$-simulator; - $\epsilon$-zero-knowledge commit-and-prove whose commit stage is extractable with $\epsilon$-simulation; - $\epsilon$-simulatable coin-flipping; - $\epsilon$-zero-knowledge arguments of knowledge for $\mathbf{NP}$ for which the knowledge extractor is also an $\epsilon$-simulator; - $\epsilon$-zero-knowledge arguments for $\mathbf{QMA}$. At the heart of the above results is a black-box extraction lemma showing how to efficiently extract secrets from QPT adversaries while disturbing their quantum state in a controllable manner, i.e., achieving $\epsilon$-simulatability of the post-extraction state of the adversary.

==> other-notes.tex <==
%!TEX root = ./main.tex

\section{Other Notes}
\xiao{Here are some notes from Kai-Min and Takashi}

Can we build a black-box $\omega(1)$-round PQ-2PC (with negligible simulation error)? If so, we get optimal round complexity for both $\epsilon$ and standard security. 
\begin{takashienv}{}
I've been thinking about a related problem to construct a black-box $\omega(1)$-round simulation-extractable commitment with negligible error from OWF. But I have no idea, and surprisingly, this seems difficult even if we rely on non-BB constructions!

On the other hand, if our goal is a black-box $\omega(1)$-round PQ-2PC with negligible error from OT, this might be feasible. The key point is that we can rely on OT for constructing simulation-extractable commitment for this purpose. The idea is to follow the idea of \cite{C:BCKM21}. 
\begin{itemize}
\item
Construct black-box $\omega(1)$-round equivocal commitment from OWF. This is already done in \cite{C:BCKM21}. Note that \cite{C:BCKM21} does not rely on a quantum construction in this part. \red{[Xiao: any commit and prove should satisfy this requirement.]}
\item
Construct black-box $\omega(1)$-round simulation-extractable and equivocal commitment from the above equivocal commitment and OT. Note that \cite{C:BCKM21} does this relying on quantum communication instead of OT. To my understanding, \cite{C:BCKM21} uses quantum communication to use CK88 quantum OT in an ad-hoc manner. So I feel that it's not surprising if we can replace quantum communication with post-quantum OT, though I haven't checked any details.
\item
Once we get simulation-extractable and equivocal commitment with negligible error, the rest is the same as our current strategy. 
\end{itemize}
\end{takashienv}





==> sections/2PC.tex <==
%!TEX root=../main.tex

\section{$\epsilon$-Simulatable 2PC}
\subsection{Definitions and a Non-Concurrent Composition Lemma}
We first present the formal definition for $\epsilon$-simulatable two-party computation. This is identical to the standard 2PC definition in the classical setting except that:
\begin{enumerate}
\item
The malicious party can be QPT;
\item
The indistinguishability between the real-world execution and the simulated one is parameterized by a function $\epsilon(\secpar) \le 1$. 
\end{enumerate}

\para{Notation.} Consider two parties $P_1$ and $P_2$ with inputs $x_1$ and $x_2$ that wish to interact in a protocol $\Prot$ to evaluate a 2-party
functionality $f$ on their joint inputs. The ideal and real executions follow the standard description as in, e.g., \cite{Goldreich04}.

In the real world, a QPT adversary $\Adv_\secpar$ with a quantum auxiliary input $\rho_\secpar$ corrupting $P_i(x_i)$ ($i\in \bits$) interacts with $P_{1-i}(x_{1-i})$. Let $\vb{x} = (x_1, x_2)$ denote the inputs to the two parties. Let $\REAL_{\Prot, \Adv, i}(\secpar, \vb{x}, \rho_\secpar)$ denote the random variable consisting of the output of the adversary (which may be an arbitrary function of its view and in particular may be a quantum state) and the outputs of the honest party $P_{1-i}$. 

In the ideal world, a QPT machine $\Sim$ controls the same party $P_i$ as $\Adv_\secpar$. It gets $x_i$ and $\rho_\secpar$ as input. Similar as in the $\epsilon$-ZK definition \cite{chia2020black}, $\Sim$ additionally takes as input a ``slackness parameter''\footnote{Actually, \cite{chia2020black} call it ``accuracy parameter''. But we think ``slackness'' is a better name as $\epsilon$ measures how {\em far} two ensembles are.} $\epsilon(\secpar) < 1$, which is a noticeable function on $\secpar$. Henceforth, we always require that $\Sim$'s running time is a polynomial on both $\secpar$ and $\epsilon^{-1}$. Let $\IDEAL_{f,\Sim,i}(\secpar, \epsilon, \vb{x}, \rho_\secpar)$ denote the outputs of $\Sim$ (with slackness $\epsilon$) and the uncorrupted party $P_{1-i}$ from the ideal-world execution.

 We remark that, throughout this paper, we only focus on {\em static} adversaries and {\em security with abortion} (i.e., the ideal-world adversary (aka the simulator) learns the its output first, and then can instruct the ideal functionality to deliver the output to the honest party or not). This is standard in 2PC literature as security without abortion (aka {\em fairness}) is impossible for {\em general-purpose} two-party protocols \cite{STOC:Cleve86,TCC:ABMO15}.

\begin{definition}[$\epsilon$-Simulatable 2PC] \label{def:e-2pc}
 Let $f$ be a 2-party functionality, and \Prot be a 2-party protocol. We say that $\Prot$ is a {\em $\epsilon$-simulatable} protocol for $f$ if there exists a QPT simulator $\Sim$ such that for any non-uniform QPT adversary $\Adv = \Set{\Adv_\secpar, \rho_\secpar}_{\secpar\in\Naturals}$, any $i \in \bits$, any $\vb{x}\in (\bits^*)^2$, and any noticeable function $\epsilon(\secpar)$, it holds that:
$$\Set{\REAL_{\Prot, \Adv, i}(\secpar, \vb{x}, \rho_\secpar)}_{\secpar \in \Naturals} ~\cind_\epsilon~ \Set{\IDEAL_{f,\Sim,i}(\secpar, \epsilon, \vb{x}, \rho_\secpar)}_{\secpar \in \Naturals}.$$
\end{definition}

\para{Non-Concurrent Composition.} We now prove a lemma that will allow us to securely compose different $\epsilon$-simulatable protocols together, as long as the composition happens in a ``non-concurrent'' (explained later) manner. This lemma is a straight-forward extension of the non-concurrent composition lemma from \cite{JC:Canetti00} to the $\epsilon$-simulatable 2PC protocols in \Cref{def:e-2pc}.

\subpara{The Hybrid Model.} We start by specifying the model for evaluating a 2-party function $g$ with the assistance of a trusted party computing some 2-party functionalities $(f_1, \ldots, f_m)$. The trusted party is invoked at special rounds, determined by the protocol. In each such round, a function $f$ (out of $f_1, \ldots, f_m$) is specified. At this point, both parties pause the execution of $\pi$, store their current state, and then start to make the call to the ideal functionality $f$. Upon receiving the output back from the trusted party, the protocol $\pi$ continues.

The protocol $\pi$ is such that $f_{i+1}$ can be called only if the invocation of $f_{i+1}$ is completely finished. It is possible that $f_i = f_j$ for some $i \ne j$, representing that the same ideal functionality is invoked twice at different time point. We emphasis that, during the invocation of some $f_i$, the honest party does not send/respond any other messages until it finishes the execution with $f_i$. This is called ``non-concurrent requirement'' in \cite{JC:Canetti00}. For an execution of $\pi$ in the $(f_1, \ldots, f_m)$-hybrid model, we use $\EXEC^{f_1, \ldots, f_m}_{\pi, \Adv, i}(\secpar, \vb{x}, \rho_\secpar)$ to denote the joint outputs of the adversary corrupting $P_i(x_i)$ and the honest $P_{1-i}(x_{1-i})$. 

Let $(\rho_1, \ldots, \rho_m)$ be ``subroutine'' protocols that are supposed to compute $(f_1, \ldots, f_m)$ respectively. We use $\pi^{\rho_1, \ldots, \rho_m}$ to denote the (plain-model) protocol obtained by replacing the ideal calls in the $(f_1, \ldots, f_m)$-hybrid protocol $\pi$ with the corresponding ``subroutine'' protocols in $(\rho_1, \ldots, \rho_m)$.

With these notations, we present the composition lemma for $\epsilon$-simulatable protocols in \Cref{lem:e-composition}. We remark that \Cref{lem:e-composition} can be generalized to $n$-party ($n>2$) setting with $m>1$ subroutines $\Set{\rho_i}_{i\in [m]}$ such that $\rho_i$ is a $\epsilon$-simulatable protocol for $f_i$, as long as the composition is non-concurrent (similar as in the original theorem \cite[Theorem 5 and Corollary 7]{JC:Canetti00}). Here, we choose to present the 2-party (i.e., $n=2$) version with only a single (i.e., $m=1$) subroutine protocol $\rho$ as this already suffices for our application.  \xiao{It turns out that we do need to prove this lemma for $m>1$... Our smOT to OT compiler works in a $\Func_\textsc{ct}$-hybrid model where the $\Func_\textsc{ct}$ functionality is invoked more than one time...} 

\begin{lemma}[Composition of $\epsilon$-Simulatable Protocols]\label{lem:e-composition}
Let $\rho$ be a $\epsilon$-simulatable protocol for a 2-party functionality $f$. Let $\pi$ be a $\epsilon$-simulatable protocol for a 2-party functionality $g$ {\em in the $f$-hybrid model}. Then, $\pi^\rho$ is a $\epsilon$-simulatable protocol for $g$.
\end{lemma}
\begin{proof}
Since $\pi$ is a $\epsilon$-simulatable protocol for $g$ in the $f$-hybrid model, there is a QPT $\Sim'$ such that for any non-uniform QPT $\Adv' = \Set{\Adv'_\secpar, \alpha_\secpar}_{\secpar\in\Naturals}$, any $i \in \bits$, any $\vb{x}\in (\bits^*)^2$, and any noticeable $\epsilon(\secpar)/2$, 
\begin{equation}\label{eq:e-composition:ideal'-hybrid}
\Set{\IDEAL_{g, \Sim', i}(\secpar, \frac{\epsilon}{2}, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals} ~\cind_{\frac{\epsilon}{2}}~ \Set{\EXEC^f_{\pi, \Adv', i}(\secpar, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals}.
\end{equation}
Now, in the LHS execution of \Cref{eq:e-composition:ideal'-hybrid}, consider a new $\Sim$ that on input $\epsilon$, it runs $\Sim'$ with slackness parameter $\epsilon/2$. Note that $\Sim$'s running time is also a polynomial on $\secpar$ and $\epsilon^{-1}$. Indeed, $\Sim$ is identical to $\Sim'$ with only syntactical changes. Thus, we have
\begin{equation}\label{eq:e-composition:ideal'-hybrid}
\Set{\IDEAL_{g, \Sim, i}(\secpar, \epsilon, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals} ~\idind~ \Set{\IDEAL_{g, \Sim', i}(\secpar, \frac{\epsilon}{2}, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals} ~\cind_{\frac{\epsilon}{2}}~ \Set{\EXEC^f_{\pi, \Adv', i}(\secpar, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals}.
\end{equation}
Therefore, \Cref{lem:e-composition}, follows from the following \Cref{claim:e-composition:hybrid-real}.
\end{proof}

\begin{myclaim}\label{claim:e-composition:hybrid-real}
Let $\rho$, $f$ and $\pi$ be the same as in \Cref{lem:e-composition}.
There exists a quantum adversary $\Adv'$ in the $f$-hybrid execution of $\pi$ such that for any non-uniform QPT $\Adv = \Set{\Adv_\secpar, \alpha_\secpar}_{\secpar\in\Naturals}$ in the real execution of $\pi^\rho$, any $i \in \bits$, any $\vb{x}\in (\bits^*)^2$, and any noticeable $\epsilon(\secpar)$, 
\begin{equation}\label{eq:e-composition:hybrid-real}
\Set{\EXEC^f_{\pi, \Adv', i}(\secpar, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals} ~\cind_{\frac{\epsilon}{2}}~ \Set{\REAL_{\pi^\rho, \Adv, i}(\secpar, \vb{x}, \alpha_\secpar)}_{\secpar \in \Naturals},
\end{equation}
where $\Adv'$'s running time is a polynomial on $\secpar$ and $\epsilon^{-1}$.
\end{myclaim}
\begin{proof}
This proof proceeds as follows:
\begin{enumerate}
\item
We construct out of $\Adv = \Set{\Adv_\secpar, \alpha_\secpar}_{\secpar\in\Naturals}$ a QPT real-world adversary $\Adv^\rho = \Set{\Adv^\rho_{\secpar}, \alpha^\rho_\secpar}_{\secpar\in\Naturals}$ that operates against protocol $\rho$ as a stand-alone protocol. The security of $\rho$ guarantees that $\Adv^\rho$ has a QPT simulator $\Sim^\rho$ such that for any $i$, $\vb{x}$, and $\epsilon/2$, 
\begin{equation}\label{eq:ideal-real:rho}
\Set{\IDEAL_{f, \Sim^\rho, i}(\secpar, \frac{\epsilon}{2}, \vb{x}, \alpha^\rho_\secpar)}_{\secpar \in \Naturals} ~\cind_{\frac{\epsilon}{2}}~ \Set{\REAL_{\rho, \Adv^\rho, i}(\secpar, \vb{x}, \alpha^\rho_\secpar)}_{\secpar \in \Naturals}.
\end{equation}
\item
Out of $\Adv$ and $\Sim^\rho$, we construct an adversary $\Adv'$ that operates against protocol $\pi$ in the $f$-hybrid model. We then finish the proof by showing that $\Adv'$ satisfies \Cref{eq:e-composition:hybrid-real} and the running time requirement.
\end{enumerate}

\subpara{The Simulator $\Sim^\rho$ for Protocol $\rho$.} We provide more details. Intuitively, $\Adv^\rho$ represents the ``segment'' of $\Adv$ that is involved in the execution of $\rho$. That is, $\Adv^\rho$ takes a non-uniform quantum auxiliary input $\Set{\alpha^\rho_\secpar}_{\secpar\in\Naturals}$. This auxiliary input contains the internal state of $\Adv$, controlling party $P_i(x_i)$, and executing the protocol $\pi^\rho$ with the honest party $P_{1-i}(x_{1-i})$ up to round $\ell_\rho$, where $\rho$ is invoked. We note that $\Set{\alpha^\rho_\secpar}_{\secpar\in\Naturals}$ can be constructed from $\Set{\alpha_\secpar}_{\secpar\in\Naturals}$ (i.e., $\Adv$'s auxiliary input). At the end of its execution of $\rho$ with $P_{1-i}(x_{1-i})$, adversary $A^\rho$ outputs the current state of the simulated $\Adv$. 

By assumption, $\rho$ is a $\epsilon$-simulatable protocol for $f$. Thus, there exists a QPT $\Sim^\rho$ satisfying \Cref{eq:ideal-real:rho}.

\subpara{$\Adv'$ in the $f$-Hybrid Model.} Adversary $\Adv'$ represents the ``segment'' of $\Adv$ that executes $\pi$ in the $f$-hybrid model, where $\Adv$'s execution of $\rho$ is handled by $\Sim^\rho$. Recall that $\Adv$ expects to execute the protocol $\pi_\rho$, not $\pi$ in the $f$-hybrid model. Therefore, we will need $\Sim^\rho$ to simulate the $\rho$ part for $\Adv$.  Formally, $\Adv'$ starts by invoking $\Adv_\secpar$ on auxiliary input $\alpha_\secpar$, and follows $\Adv$'s instructions up to round $\ell_\rho$.
At this point, $\Adv$ expects to execute $\rho$ with $P_i$, whereas $\Adv'$ invokes the ideal functionality $f$ (of the $f$-hybrid model). To continue the execution of $\Adv$, adversary $\Adv'$ runs $\Sim^\rho$. For this purpose, $\Sim^\rho$ is given the auxiliary input, denoted as $\alpha^\rho_\secpar$, that describes the current state of $\Adv$ at round $\ell_\rho$. The information from $\Sim^\rho$'s trusted party is emulated by $\Adv'$, using $\Adv'$'s own ideal functionality $f$. Recall that the output of $\Sim^\rho$ is a (simulated) internal state of $\Adv$ at the completion of protocol $\rho$. Once protocol $\rho$ completes its execution and the parties return to running $\pi$, adversary $\Adv'$ returns to running $\Adv$ (starting from the state in $\Sim^\rho$'s output) and follows the instructions of $\Adv$. When $\Adv$ terminates, $\Adv'$ outputs whatever $\Adv$ outputs.

With $\Adv'$ defined above, the LHS and RHS executions of \Cref{eq:e-composition:hybrid-real} can be divided into the following 3 stages:
\begin{enumerate}
\item \label[Stage]{stage:e-composition:hybrid-real-1}
Both the LHS and RHS executions are identical up to the starting of round $\ell_\rho$
\item \label[Stage]{stage:e-composition:hybrid-real-2}
At round $\ell_\rho$, the RHS $\Adv$ starts executing $\rho$ with the honesty $P_{1-i}$, whereas the LHS $\Adv$ (controlled by $\Adv'$) talks with $\Sim^\rho$. At the end of this stage, the internal state of $\Adv$ in the RHS is $\epsilon/2$-far from the ($\Sim^\rho$-simulated) internal state of $\Adv$ (controlled by $\Adv'$) in the LHS. 
\item \label[Stage]{stage:e-composition:hybrid-real-3}
Then, both the LHS and RHS again proceed identically until the end. 
\end{enumerate} 
Since both \Cref{stage:e-composition:hybrid-real-1,stage:e-composition:hybrid-real-3} are polynomial time, \Cref{eq:e-composition:hybrid-real} follows from a straightforward reduction to the $\epsilon$-simulatability of $\Sim^\rho$ in \Cref{stage:e-composition:hybrid-real-2} (by setting the slackness parameter to $\epsilon/2$).

Finally, we need to argue that $\Adv'$'s running time is a polynomial on $\secpar$ and $\epsilon'$. This is true as $\Adv'$ does nothing more than running $\Adv$ and $\Sim^\rho$, and both of them is QPT on $\secpar$ and $\epsilon$. (Though $\Sim^\rho$ is invoked with slackness $\epsilon/2$, $(\epsilon/2)^{-1}$ is also a polynomial on $\epsilon^{-1}$.) 
\end{proof}

\subsection{Black-Box $\epsilon$-Simulatable 2PC in Constant Rounds}
In this part, we construct a $\epsilon$-Simulatable 2PC. Concretely, we establish the following theorem.

\begin{xiaoenv}{$\epsilon$-smOT or standard smOT?}
In \Cref{thm:e-2pc:main}, we need to decide if we want to assume $\epsilon$-smOT or standard smOT. It seems we need to assume smOT as the \cite{TCC:Haitner08} compiler uses it. Then, there are two choices:
\begin{itemize}
\item
Assume smOT directly. This is ok since we have so many constructions. However, if we want to do this, we should also show that $\epsilon$-smOT in the minimal assumption for $\epsilon$-2PC. (this proof has not appeared before.)
\item
Assume $\epsilon$-smOT and seek to prove that ``$\epsilon$-smOT implies $\epsilon$-2PC''. The only extra thing (in addition to the \cite{STOC:IKLP06,TCC:Haitner08} compiler) is to prove that $\epsilon$-smOT implies smOT. This seems possible to achieve.
\end{itemize}
\end{xiaoenv}
\begin{theorem}[Black-Box Constant-Round $\epsilon$-2PC]\label{thm:e-2pc:main}
Assume the existence of $\epsilon$-simulatable semi-honest oblivious transfers ($\epsilon$-smOTs). Then, for every well-formed 2-party functionality $\Func$, there exists a $\epsilon$-simulatable protocol $\Prot_\Func$. Moreover, $\Prot_\Func$ only makes black-box access to the $\epsilon$-smOT; if $\epsilon$-smOT is in constant rounds, $\Prot_\Func$ will also be in constant rounds.   
\end{theorem}
\xiao{Say that $\epsilon$-smOTs are know from both generic and algebraic assumptions (i.e., LWE/Isogeny/LPN with some parameter setting?). Give some exemplary citations.... [Important:] need to show that the semi-honest security of these constructions holds against QPT adversaries.}



\begin{proof}
This proof consists of the following two steps:
\begin{enumerate}
\item \label[Step]{item:e-2pc:main:proof:step-1}
Construct a $\epsilon$-simulatable maliciously-secure OT ($\epsilon$-OT) by making black-box use of $\epsilon$-smOT and incurring only a constant number of extra rounds. 
\item \label[Step]{item:e-2pc:main:proof:step-2}
Construct the $\Prot_\Func$ in \Cref{thm:e-2pc:main} by  making black-box use of $\epsilon$-OT and incurring only a constant number of extra rounds. 
\end{enumerate}

\subpara{For \Cref{item:e-2pc:main:proof:step-2}.} We first deal with \Cref{item:e-2pc:main:proof:step-2} as it is simpler. Our starting point is the constant-round black-box universally-composable (UC) MPC protocol by Ishai, Prabhakaran, and Sahai \cite[Section 5.2]{C:IshPraSah08} (henceforth, IPS) in the OT-hybrid model. As a vigilant reader may have noticed already, the security of the IPS protocol was proved against classical polynomial-time adversaries, whereas we need it to be secure against QPT adversaries. However, as already observed in previous work (e.g., \cite{EC:Unruh10,DBLP:conf/eurocrypt/AgarwalBGKM21}), the IPS protocol is indeed secure against QPT adversaries in the OT-hybrid model, because the simulator does not rewind or clone the adversary's state. Therefore, in the OT-hybrid model, the (2-party version of) IPS protocol computes $\Func$ securely against QPT adversaries. Thus, it is of course a $\epsilon$-simulatable protocol for $\Func$ in the OT-hybrid model. Finally, the $\Prot_\Func$ in \Cref{item:e-2pc:main:proof:step-2} can be constructed by replacing the ideal-function OT with the $\epsilon$-OT protocol in the IPS construction and invoking \Cref{lem:e-composition}. 	

Here is one more caveat: the IPS protocol also makes black-box use of PRGs (in addition to the OT). This assumption was usually not stated explicitly because it is well-known that smOTs imply PRGs in a black-box manner. However, in the current proof, we only have a $\epsilon$-smOT. This is actually not a problem as $\epsilon$-smOTs also imply PRGs in a black-box manner---\xnote*{@CCY: please verify this claim.}{it is not hard to see that $\epsilon$-smOTs imply the existence of weak OWFs\footnote{That is, the slackness in one-wayness is only $1/\poly$, instead of negligible.}}. Weak OWFs can be ``amplified'' to standard OWFs using XOR lemmas \cite{FOCS:Yao82a,DBLP:journals/combinatorica/Levin87,FOCS:Impagliazzo95,DBLP:books/sp/goldreich2011/GoldreichNW11}, which then give rise to a PRG in black-box \cite{STOC:GolLev89,STOC:ImpLevLub89,HILL99}.
\takashi{Is it clear that the amplification works against quantum adversaries? But I think this argument could be avoided here since I believe $\epsilon$-smOT implies (not weak) OWF. Namely, the OWF is the function that maps a randomness to the corresponding transcript. If an adversary can invert it with non-neg probability $\delta$, then this would contradict $\epsilon$-simulation security since $\epsilon$ can be arbitrarily small inverse-poly and in particular can be smaller than $\delta$.} 

\subpara{For \Cref{item:e-2pc:main:proof:step-1}.} We start with the constant-round compiler transferring smOTs to OTs in the classical setting \cite{STOC:IKLP06,TCC:Haitner08,DBLP:journals/siamcomp/HaitnerIKLP11} (henceforth, HIKLP). The HIKLP compiler makes only black-box use of the smOT protocol and additionally a coin-tossing protocol. In other words, this compiler can be interpreted as a protocol $\Prot_\textsc{hiklp}$ that securely compute the OT functionality $\Func_\textsc{ot}$ in the $\Func_\textsc{ct}$-hybrid model, where $\Func_\textsc{ct}$ is the ideal functionality for coin-tossing.

Ideally, if the security proof for $\Prot_\textsc{hiklp}$ in the $\Func_{ct}$-hybrid model works against QPT adversaries (just as the IPS protocol above), then we can finish the current proof by instantiating the $\Func_\textsc{ct}$ with a $\epsilon$-simulatable coin-tossing and invoking \Cref{lem:e-composition} (similar as what we did for \Cref{item:e-2pc:main:proof:step-2}). However, it is not clear if $\Prot_\textsc{hiklp}$ is secure against QPT adversaries! In particular, there are two places in the classical security proof (i.e., against PPT adversaries) for $\Prot_\textsc{hiklp}$ where rewinding is necessary. 

To address this issue, we prove that the $\Prot_\textsc{hiklp}$ \xiao{see if slight modification is needed} compiler is indeed secure against QPT adversaries in the $\Func_{ct}$-hybrid model (w.r.t.\ the $\epsilon$-simulatable security). That is, we will establish the following lemma, which we will prove in \Cref{sec:smOT-OT}.
\begin{lemma}[Black-Box $\epsilon$-Simulatable OT]\label{lem:epsilon-HIKLP}
Assuming the existence of semi-honest OTs secure against QPT adversaries. Then, the $\Prot_\textsc{hiklp}$ compiler is a $\epsilon$-simulatable protocol for $\Func_\textsc{ot}$ in the $\Func_\textsc{ct}$-hybrid model. Same as in the classical setting, the $\Prot_\textsc{hiklp}$ compiler only makes black-box use of the semi-honest OT and incurs a constant number of extra rounds. 
\end{lemma}

Recall that we also need to instantiate the $\Func_\textsc{ct}$ functionality. To do that, we establish the following lemma, whose proof will appear in \Cref{sec:epsilon-ct}.

\begin{lemma}[Black-Box $\epsilon$-Simulatable Coin-Tossing]\label{lem:epsilon-ct}
Assuming the existence of OWFs secure against QPT adversaries. Then, there exists a $\epsilon$-simulatable protocol $\Prot_\textsc{ct}$ for $\Func_\textsc{ct}$. Moreover, $\Prot_\textsc{ct}$ only makes black-box use of the OWF and has a constant number of rounds. 
\end{lemma}

In summary, to finish \Cref{item:e-2pc:main:proof:step-1}, we first use \Cref{lem:epsilon-HIKLP} to convert the semi-honest OT to a $\epsilon$-simulatable OT in the $\Func_\textsc{ct}$-hybrid model; then, we instantiates the ideal $\Func_\textsc{ct}$ functionality via the $\Prot_\textsc{ct}$ protocol from \Cref{lem:epsilon-ct}. This leads to a $\epsilon$-simulatable OT in the plain model because of \Cref{lem:e-composition}. This construction makes only black-box use of semi-honest OTs (note that semi-honest OTs implies OWFs); it has a constant number of rounds if the semi-honest OT does so.

This finishes the proof of \Cref{thm:e-2pc:main}.
\end{proof}


\section{Black-Box OTs from Semi-Honest OTs: the Post-Quantum Setting}
\label{sec:smOT-OT}
\begin{xiaoenv}{HIKLP Road map}
\begin{itemize}
\item
talk about the HIKLP road map: psmOT $\rightarrow$ dS-dS $\rightarrow$ dS-mR $\rightarrow$ mS-dR $\rightarrow$ mS-mR.
\item
highlight the quantum-problematic step. Maybe, a diagram will help.
\end{itemize}
Say that the compiler here is general---we could have potentially followed HIKLP to talk about general 2PC protocols. But here to focus on OTs.
\end{xiaoenv}

\begin{remark}[On String OTs]\label{remark:string-OTs}
Throughout this work, we only focus on $\binom{2}{1}$ {\em bit} OTs, instead of {\em string} OTs. This is w.l.o.g.\ because, as pointed out by \cite{C:IshPraSah08}, there are efficient and unconditionally UC-secure reductions with constant communication overhead from $\binom{N}{1}$ string OTs to $\binom{2}{1}$ bit OTs (implicit in \cite{C:Crepeau87,DBLP:journals/tit/BrassardCS96,C:DodMic00,EC:CreSav06}). \xiao{This could be problematic as we need such a reduction in the plain model....}
\end{remark}
\subsection{Various Security Notions for OT}

\para{Semi-Honest Private OTs.} This primitive is weaker than the standard semi-honest OTs, as it does not  require the existence of even {\em semi-honest} simulators. Instead, it simply requires that after the execution of an OT protocol between two {\em honest} parties, each party does not learn anything (in an indistinguishability-based sense) about the information he is not supposed to learn.
\begin{definition}[Semi-Honest Private OTs \cite{DBLP:journals/siamcomp/HaitnerIKLP11}]\label{def:psm-ot}
A two-party protocol $\Prot = (S,R)$ is a semi-honest private OT (psm-OT) if it satisfies the natural completeness requirement and the following security requirements:
\begin{itemize}
\item {\bf Privacy against semi-honest senders:} for every input $(s_0, s_1) \in \bits \times \bits$ for the sender, it holds that:
\begin{equation}\label{eq:def:psm:receiver}
\Set{\View_S\langle S(1^\secpar, (s_0,s_1)), R(1^\secpar, r) \rangle, r}~\cind~\Set{\View_S\langle S(1^\secpar, (s_0,s_1)), R(1^\secpar, r)\rangle, r' },
\end{equation}
where $r$ and $r'$ are independent samples drawn uniformly from $\bits$.

\item {\bf Privacy against semi-honest receivers:} for every input $r \in \bits$ for the receiver, it holds that:
\begin{equation}\label{eq:def:psm:sender}
\Set{\View_R\langle S(1^\secpar, (s_0,s_1)), R(1^\secpar, r) \rangle, s_{1-r}}~\cind~\Set{\View_R\langle S(1^\secpar, (s_0,s_1)), R(1^\secpar, r) \rangle , s'_{1-r}},
\end{equation}
where $s_0$, $s_1$ and $s'_{1-r}$ are independent samples drawn uniformly from $\bits$.
\end{itemize}
\end{definition}


\xiao{Prove a lemma here: $\epsilon$-OT against semi-honest adversaries is always semi-honest private OT as per \Cref{def:psm-ot}.}

\para{Defensibly Private OTs.} This notion upgrades the previous semi-honest privacy by allowing malicious QPT adversaries. However, at the end of the execution, the malicious party is required to output a ``defense''\footnote{W.l.o.g., one can assume that the defense always appears in some pre-defined position of the adversary's output, e.g., the last chunk of its view.} that can explain its behavior as an honest party during the execution. We recall the definition of a good defense in the following.
\begin{definition}[A Good Defense \cite{DBLP:journals/siamcomp/HaitnerIKLP11}]
 Let $t$ be the transcript of an execution of an $\mathsf{N}$-round protocol $\Prot = (P_1, P_2)$ between an adversary $\Adv$ (say, controlling $P_1$) and the honest party (say $P_2$). Then, we say that the pair $(x_1, \gamma_1)$ constitutes {\em a good defense} by $\Adv$ for $t$ in $\Prot$, if for every $\ell \in \mathsf{N}$ it holds that $\algo{sent}^{\Adv}_\ell(t) = P_1\big(x_1, \gamma_1; \algo{received}^\Adv_{1, \ldots, \ell-1}(t)\big)$, where $\algo{sent}^{P_i}_\ell(t)$ denotes the $\ell$-th message sent by $P_i$ in $t$, and $\algo{received}^{P_i}_{1, \ldots, \ell-1}(t)$ denotes the first $\ell$ messages received by $P_i$ in $t$.
\end{definition}
An invalid defense can be interpreted as the adversary admitting that she is cheating. In that case, we do not require any security; However, as long as the defense is valid, we hope that the adversary can do no harm (in terms of \Cref{def:psm-ot}). This is formalized as follows.
\begin{definition}[Defensibly Private OTs \cite{DBLP:journals/siamcomp/HaitnerIKLP11}]\label{def:dp-ot}
A two-party protocol $\Prot = (S,R)$ is a defensibly private OT (pd-OT) if it satisfies the natural completeness requirement and the following security requirements:
\begin{itemize}
\item {\bf Privacy against defensible senders:} Let $\Gamma_S(\cdot, \cdot)$ be a function such that $\Gamma_S(v,*) = (v, *)$ if $v$ contains a valid sender's defense; otherwise, $\Gamma_S(v, *)=(\bot, \bot)$. For any non-uniform QPT sender $\Set{S^*_\secpar, \rho_\secpar}_{\secpar \in \Naturals}$, it holds that:
\begin{equation}\label{eq:def:dp:receiver}
\big\{\Gamma_S\big(\View_{S_\secpar^*}\langle S_\secpar^*(\rho_\secpar), R(1^\secpar, r) \rangle, r\big)\big\}~\cind~\big\{\Gamma_S\big(\View_{S_\secpar^*}\langle S_\secpar^*(\rho_\secpar), R(1^\secpar, r) \rangle, r'\big)\big\},
\end{equation}
where $r$ and $r'$ are independent samples drawn uniformly from $\bits$.

\item {\bf Privacy against defensible receivers:} Let $\Gamma_R(\cdot, \cdot)$ be a function such that $\Gamma_R(*,v) = (*,v)$ if $v$ contains a valid receiver's defense; otherwise, $\Gamma_R(*,v)=(\bot, \bot)$. For any non-uniform QPT receiver $\Set{R^*_\secpar, \rho_\secpar}_{\secpar \in \Naturals}$, it holds that:
\begin{equation}
\big\{\Gamma_R\big(\View_{R^*_\secpar}\langle S(1^\secpar, (s_0,s_1)), R^*_\secpar(\rho_\secpar) \rangle, s_{1-r}\big)\big\}~\cind~\big\{\Gamma_R\big(\View_R\langle S(1^\secpar, (s_0,s_1)), R^*_\secpar(\rho^\secpar)\rangle, s'_{1-r}  \big)\big\},
\end{equation}
where the $r$ is the receiver's input contained in $R^*$'s (valid) defense, the $s_0$, $s_1$ and $s'_{1-r}$ are independent samples drawn uniformly from $\bits$.
\end{itemize}
\end{definition}

\xiao{need to talk about the standard fully-simulatable OT.}

\para{Notation.} Henceforth, we use \psms (resp.\ \psmr) to denote an OT achieving privacy against semi-honest sender's (resp.\ receivers); \pds (resp.\ \pdr) refers to OTs achieving privacy against defensible sender's (resp.\ receivers); \es (resp.\ \er) refers to OTs achieving the $\epsilon$-simulatable security against malicious senders (resp.\ receivers). In particular, \psms-\psmr OTs (resp.\ \pds-\pdr OTs) are OTs satisfying \Cref{def:psm-ot} (resp.\ \Cref{def:dp-ot}); we will also refer to hybrid ones such as \psms-\pdr OTs or \pds-\er OTs, whose meanings should be self-evident from their names.


\subsection{From Semi-Honest Privacy to Defensible Privacy}
We show a constant-round black-box compiler that converts semi-honest privacy OTs to defensibly private OTs. Our compiler shares a similar structure as that in \cite{DBLP:journals/siamcomp/HaitnerIKLP11}. But the security proof is very different. That is because the \cite{DBLP:journals/siamcomp/HaitnerIKLP11} compiler relies on a rewinding analysis which is hard (if not impossible) to migrate to the post-quantum setting. %We provide more details in the following.

\subsubsection{Privacy against Defensible Senders} 
\label{sec:achieving-pdS}
To illustrate the idea, let us first focus on receiver's privacy (i.e., against adversarial senders). That is, we show how to compiler a \psms-\psmr OT to a \pds-\psmr OT. This compiler is ``symmetric'' in the sense that applying it again on the receiver's side of the \pds-\psmr OT will eventually yield the desired \pds-\pdr OT. We will discuss the second step in \Cref{sec:achieving-pdR}.


At a high-level, the compiler works by asking the (potentially-malicious) sender to commit to its input and a random string at the beginning. Then, the two parties execute the psm-OT protocol, where the sender is supposed to use the committed input and random string (as its randomness) when executing the psm-OT. Intuitively, this ensures receiver's privacy against defensible senders because:
\begin{enumerate}
\item
If the sender behaves in the psm-OT like an honest sender with the input and random tape committed earlier, then the receiver's privacy follows from the security of psm-OT (against semi-honest senders).
\item
The sender has no choice but to use the input and randomness committed earlier, as otherwise it cannot give a valid defense at the end of the execution.
\end{enumerate} 
Formalizing the above idea requires caution. Concretely, given a malicious sender-distinguisher pair $(S^*_\pd, D_\pd)$ breaking the receiver's defensible privacy, we want to build a distinguisher\footnote{Recall that semi-honest privacy OTs considers only semi-honest parties. So, there is no ``adversarial sender''.} $D_\psm$ that breaks the receiver's semi-honest privacy. That is, $D_\psm$ takes as input either the LHS or RHS of \Cref{eq:def:psm:receiver} and tries to distinguish. As one can imagine, $D_\psm$, on its input from the external \psm-OT challenger (against semi-honest senders), will run $S^*_\pd$ internally, simulate the \psm-OT execution in some particular way, and finally invoke $D_\pd$. However, $D_\psm$ cannot choose the randomness used by the semi-honest sender in the \psm-OT game; this randomness is given to $D_\psm$ as a part of $\View_S\langle S(1^\secpar, (s_0,s_1)), R(1^\secpar, r)\rangle$ from the external challenger. In contrast, $S^*_\pd$ is not necessarily semi-honest and can choose its random tap (to commit at the beginning) that it will use in the later \psm-OT execution. Therefore, it is unclear how $D_\psm$ can make use of $S^*_\pd$. 

\cite{DBLP:journals/siamcomp/HaitnerIKLP11} resolved this issue by asking the receiver to contribute a share to $S^*_\pd$'s randomness used in the \psm-OT stage. In more details, the receiver sends random string after $S^*_\pd$'s first commitment; then, $S^*_\pd$ is required to use the XOR of receiver's random string and the committed random tape as its randomness in the \psm-OT execution. In this way, by selecting the proper receiver's message, $D_\psm$ can ``equivocate'' $S^*_\pd$'s randomness tape when simulating the \psm-OT execution internally, to make it match the randomness in the semi-honest sender's view (from the \psm-OT challenger). To equivocate it to the desired random tape, $D_\psm$ actually needs to extract the share $S^*_\pd$ committed at the beginning, which necessarily requires rewinding. In summary, the \cite{DBLP:journals/siamcomp/HaitnerIKLP11} $D_\psm$ takes the following two-phase form:
\begin{itemize}
\item {\bf Learning phase:}
it first simulates $\pd$-OT between $S^*_\pd$ and an honest receiver (who uses fresh randomness each time) for several times, trying to extract the random share committed by $S^*_\pd$ at the beginning (from the valid defense output by $S^*_\pd$ at the end of a successful execution);
\item {\bf Predicting phase:}
 it then performs the main simulation by setting the receiver's share of randomness such that its XOR with the $S^*_\pd$'s share extracted above equals the randomness in the semi-honest sender's view from the external challenger.
\end{itemize} 
 % Moreover, there is one more subtlety---$S^*_\pd$'s decision in the \psm-OT execution can now depend on the receiver's share of randomness.
Migrating the above proof\footnote{We remark that the proof in \cite{DBLP:journals/siamcomp/HaitnerIKLP11} is more actually involved as the authors assume that $S^*_\pd$'s commitment is only computationally binding. Because of that, a delicate analysis is needed to ensure that $S^*_\pd$ will decommit {\em consistently} in the learning phase and predicting phase. That proof can be simplified assuming the commitment is statistically binding.} to the post-quantum setting is not trivial---rewinding a (non-uniform) QPT $S^*_\pd$ as in the above learning phase could disturb $S^*_\pd$'s quantum state too much such that one can no longer execute the predicting phase. 

This problem could be solved using the $\epsilon$-simulation-extraction lemma from \cite{chia2020black}. However, we instead take an alternative approach that admits a simpler and more modular security proof. Our idea is to replace the sender's first commitment with the $\epsilon$-simulation-extractable commitment from \Cref{sec:sim-ext-com}. With this modification, $D_\psm$ can extract the input and randomness committed by $S^*_\pd$ while disturbing its quantum state in a controllable way (i.e., at most $\epsilon$-far from its original state), and then finishes the predicting phase as before. We present the construction in \Cref{protocol:pdS-psmR-OT} and establish its security in \Cref{thm:pdS-psmR-OT}.

\begin{ProtocolBox}[label={protocol:pdS-psmR-OT}]{Oblivious Transfer $\Prot_{\psmr}^{\pds}$}
{\bf Sender's Input:} security parameter $1^\secpar$, two bits $(s_0, s_1) \in \bits \times \bits$, and randomness $\gamma_S=(\gamma^1_S, \gamma^2_S)$.\\[-1em]

{\bf Receiver's Input:} security parameter $1^\secpar$, a bit $r \in \bits$, and randomness $\gamma_R=(\gamma^1_R, \gamma^2_R, \gamma^3_R)$.
\begin{enumerate}
\item
$S$ and $R$ executes \algo{SECom} where $S$ commits to $(s_0, s_1, \gamma^2_S)$; the parties use security parameter $1^\secpar$, and random coins $\gamma^1_S$ and $\gamma^1_R$, respectively.
\item
$R$ sends $\gamma^3_R$ to $S$.
\item
$S$ and $R$ execute protocol $\Prot^{\psms}_\psmr$, where $S$ runs the sender with security parameter $1^\secpar$, input $(s_0, s_1)$, and random tape $\gamma^2_S \xor \gamma^3_R$, and $R$ runs the receiver with security parameter $1^\secpar$, input $r$, and random tape $\gamma^2_R$.
\item
$S$ (resp.\ $R$) outputs whatever the sender (resp.\ receiver) of $\Prot^{\psms}_\psmr$ outputs. 
\end{enumerate}
\end{ProtocolBox}

\begin{theorem}\label{thm:pdS-psmR-OT}
Assume that $\algo{SECom}$ is a $\epsilon$-simulation-extractable commitment satisfying \Cref{def:epsilon-simext-com} and $\Prot^\psms_{\psmr}$ is a semi-honest private OT satisfying \Cref{def:psm-ot}. Then, \Cref{protocol:pdS-psmR-OT} is an \pds-\psmr OT (i.e., achieving privacy against defensible QPT senders as per \Cref{eq:def:dp:receiver} and semi-honest receivers as per \Cref{eq:def:psm:sender}).
\end{theorem}

\subsubsection{Proof of \Cref{thm:pdS-psmR-OT}}
\begin{xiaoenv}{Proving \Cref{thm:pdS-psmR-OT}}
say that completeness follows straightforwardly. 

prove that the compiler retains the privacy against semi-honest receivers. 

then, the main proof
\end{xiaoenv}

\subsubsection{Privacy against Defensible Receivers}
\label{sec:achieving-pdR}
Recall that our eventual goal is to compile a \psms-\psmr OT to a \pds-\pdr OT. \Cref{thm:pdS-psmR-OT} only gives a \pds-\psmr OT, which we still need to upgrade to obtain privacy against defensible receivers. This can be done by simply re-use the same trick in \Cref{protocol:pdS-psmR-OT} but on the receiver's side. That is, we ask the receiver to commit to its input and a random string, and then execute \Cref{protocol:pdS-psmR-OT} using the committed input and randomness. Privacy against defensible receivers can then be proven in the same manner as in \Cref{thm:pdS-psmR-OT}. Here is one caveat---since we reuse the compiler with \Cref{protocol:pdS-psmR-OT} as the underlying OT, we need to argue that the compiler maintains the \pds security of \Cref{protocol:pdS-psmR-OT}. Fortunately, this follows from a rather standard argument. We present this construction in \Cref{protocol:pdS-pdR-OT} and establish its security in \Cref{thm:pdS-pdR-OT}.


\begin{ProtocolBox}[label={protocol:pdS-pdR-OT}]{Oblivious Transfer $\Prot_{\pdr}^{\pds}$}
{\bf Sender's Input:} security parameter $1^\secpar$, two bits $(s_0, s_1) \in \bits \times \bits$, and randomness $\gamma_S=(\gamma^1_S, \gamma^2_S, \gamma^3_S)$.\\[-1em]

{\bf Receiver's Input:} security parameter $1^\secpar$, a bit $r \in \bits$, and randomness $\gamma_R=(\gamma^1_R, \gamma^2_R)$.
\begin{enumerate}
\item
$S$ and $R$ executes \algo{SECom} where $R$ commits to $(r, \gamma^2_R)$; the parties use security parameter $1^\secpar$, and random coins $\gamma^1_S$ and $\gamma^1_R$, respectively.
\item
$S$ sends $\gamma^3_S$ to $R$.
\item
$S$ and $R$ execute protocol $\Prot^{\pds}_\psmr$ (\Cref{protocol:pdS-psmR-OT}), where $S$ runs the sender with security parameter $1^\secpar$, input $(s_0, s_1)$, and random tape $\gamma^2_S$, and $R$ runs the receiver with security parameter $1^\secpar$, input $r$, and random tape $\gamma^2_R \xor \gamma^3_S$.
\item
$S$ (resp.\ $R$) outputs whatever the sender (resp.\ receiver) of $\Prot^{\pds}_\psmr$ outputs. 
\end{enumerate}
\end{ProtocolBox}
\begin{theorem}\label{thm:pdS-pdR-OT}
Assume that $\algo{SECom}$ is a $\epsilon$-simulation-extractable commitment satisfying \Cref{def:epsilon-simext-com} and $\Prot^\pds_{\psmr}$ is a \pds-\psmr OT. Then, \Cref{protocol:pdS-pdR-OT} is an \pds-\pdr OT satisfying \Cref{def:dp-ot}.
\end{theorem}
\begin{proof}
\xiao{Say that completeness is straightforward; and \pdr can be proven following the same argument in \Cref{thm:pdS-psmR-OT}. We only need to show that it maintains the \pds security.}

\end{proof}












% \begin{xiaoenv}{Takashi's outline for this proof}
% Let $\Pi$ be a semi-honest OT and $\Pi'$ be the sender-defensible version that works as follows:
% \begin{enumerate}
% \item
% S commits to its input $x_1$ and randomness $r_1$
% \item
% R sends randomness $r_2$
% \item
% S and R jointly run $\Pi$ where S uses $r_1 \xor r_2$ as randomness.
% \end{enumerate}
% We want to prove that $\Pi'$ is secure against defensible senders. Let $S^*$ be a defensible adversary against $\Pi'$. Let's consider the following real experiment:

% \subpara{Real:}
% \begin{enumerate}
% \item
% $S^*$ sends a commitment com.
% \item
% R sends randomness $r_2$.
% \item
% $S^*$ and R jointly run $\Pi$ where R randomly chooses its input.
% \item
% $S^*$ decommits com.
% \item
% If the decommitment is valid and consistent to the transcript of $\Pi$, the experiment outputs the final state of $S^*$ and R's input. Otherwise, output $\bot$.
% \end{enumerate}
% Next, we consider the following hybrid using the CCY extraction lemma. The difference is that we add ``the extraction step'' 1.5 and $S^*$'s state and let the experiment abort if the extracted decommitment does not match that output by $S^*$ in Step 5. 

% \subpara{Hybrid 1:}
% \begin{enumerate}
% \item
%  $S^*$ sends a commitment com.
%  \begin{itemize}
%  \item {\bf Step 1.5:} We run the CCY extractor where the combination of Step 2, 3, and 4 is seen as $A_{open}$ and $S^*$'s state after Step 1 is seen as $\rho_{st}$. The extractor outputs the decommitment of com along with a simulated $S^*$'s state $\rho_{ext}$. In the next invocation of $S^*$ Step 3, its internal state starts from $\rho_{ext}$.
%  \end{itemize}

% \item
%  R sends randomness $r_2$.
% \item
% $S^*$ and R jointly run $\Pi$ where R randomly chooses its input.
% \item
% $S^*$ decommits com.
% \item
%  If the decommitment is valid, {\bf equal to the extracted one}, and consistent to the transcript of $\Pi$, the experiment outputs the final state of $S^*$ and R's input. Otherwise, output $\bot$.
% \end{enumerate}
% The epsilon-indistinguishability between Real and Hybrid 1 is clear from CCY. 

% \subpara{Hybrid 2:} In the next hybrid $\Hyb_2$, in Step 2, we program $r_2 \coloneqq r_1 \xor r_S$ where $r_1$ is the committed sender's randomness taken from the extracted decommitment and $r_S$ is a fresh randomness. Hybrids 1 and 2 are perfectly indistinguishable since $r_2$ is just a uniform string in both hybrids.

% \subpara{Hybrid 3:} In the next hybrid $\Hyb_3$, in Step 5, R's input is replaced with a random bit. I believe this can be reduced to the semi-honest security of $\Pi$ because $S^*$ has to use the randomness $r_S$ in Step 3 or otherwise the experiment's output is replaced with $\bot$.

% Then, we can complete the proof by making similar modifications from Real to $\Hyb_2$ in the reversed order.

% The game hop from $\Hyb_2$ to $\Hyb_3$ may require a more careful analysis, but I believe this should work. 
% \end{xiaoenv}

\subsection{From Defensible Privacy to $\epsilon$-Simulatable Security}

\xiao{talk about the road map}
\subsubsection{$\epsilon$-Simulatable Security against Malicious Receivers}

\xiao{show how to convert \pds-\pdr OTs to \pds-\er OTs.}

\subsubsection{OT Reverser}
% With some simple pre-processing and post-processing, 
The OT reverser from \cite{EC:WolWul06} allows two parties to run the OT with switched role. As mentioned earlier, we will use this protocol to convert a \pds-\er OT to a \es-\pdr OT. We present it as \Cref{protocol:eS-pdR-OT} and analyze its security by \Cref{thm:eS-pdR-OT}.

\begin{ProtocolBox}[label={protocol:eS-pdR-OT}]{Oblivious Transfer $\Prot_{\pdr}^{\es}$ via OT Reverser}
{\bf Inputs:} Both parties take $1^\secpar$ as the common input; $S$ takes as input two bits $(s_0, s_1) \in \bits \times \bits$; $R$ takes as input a bit $r \in \bits$.
\begin{enumerate}
\item
$S$ and $R$ run protocol $\Prot^\pds_\er$ (\red{Cref to the protocol in the previous section}) in the following way:
\begin{itemize}
\item 
$S$ plays the receiver in $\Prot^\pds_\er$ with input $\tilde{r} = s_0 \xor s_1$;
\item
$R$ samples a random bit $z \pick \bits$ and plays the sender in $\Prot^\pds_\er$ with input $\tilde{s}_0 = z$ and $\tilde{s}_1 = z \xor r$.
\end{itemize}
At the end, $S$ learns $\tilde{s}_{\tilde{r}}$ as output.
\item
$S$ sends $R$ the bit $\alpha = s_0 \xor \tilde{s}_{\tilde{r}}$.
\item
$R$ outputs $s_r = z \xor \alpha$.
\end{enumerate}
\end{ProtocolBox}

\begin{theorem}\label{thm:eS-pdR-OT}
If $\Prot^\pds_\er$ is a \pds-\er OT, then \Cref{protocol:eS-pdR-OT}  is a \es-\pdr OT.
\end{theorem}
\begin{proof}
\xiao{The classical proof (\cite[Claim 5.2]{DBLP:journals/siamcomp/HaitnerIKLP11}) carries to the post-quantum setting without modification.}
\end{proof}

\subsubsection{$\epsilon$-Simulatable Security against Malicious Senders}



\xiao{to do...}

==> sections/CoinTossing.tex <==
%!TEX root=../main.tex

\section{$\epsilon$-Simulatable Coin-Tossing}
\label{sec:epsilon-ct}
In this section, we present a $\epsilon$-simulatable parallel coin-tossing protocol. Our construction is constant-round and makes only black-box use of OWFs that are secure against PQT adversaries.

\xiao{Say that this gives us constant-round BB $\epsilon$-2PC in next section. Also, describe the road map of this section.}

\subsection{Equivocal Extractable Commitments}

\xiao{to do..}

==> sections/additional-prelim.tex <==
%!TEX root = ../main.tex
\section{Additional Preliminaries}
\subsection{Serfling's Inequality}

This {\em two-sided} version of Serfling's inequality are taken from \cite{C:BouFeh10}. 
\begin{lemma}[Serfling's Inequality {\cite{serfling1974probability,C:BouFeh10}}]\label{lem:Serfling}
Let $\vb{b} \in \bits^n$ be a bit string with $\mu\cdot n$ non-zero bits (i.e., a $\mu$-fraction is 1's). Let the random variables
$(Y_1,Y_2,\ldots,Y_k)$ be obtained by sampling $k$ random entries from $\vb{b}$ {\em without replacement}. Let $\bar{Y} \coloneqq \frac{1}{k}\sum_i^k Y_i$. Then, for any $\delta >0$, it holds that
$$\Pr[|\bar{Y} - \mu| >\delta]\le 2\exp(\frac{-2\delta^2kn}{n-k+1}).$$ 
\end{lemma}

\subsection{Verifiable Secret Sharing Schemes}\label{add-prelim:VSS}
%\xiao{The following definition for VSS com is copied from \cite{FOCS:GLOV12}}
We present in \Cref{def:VSS} the definition for verifiable secret sharing (VSS) schemes \cite{FOCS:CGMA85}. We remark that \cite{STOC:BenGolWig88,EC:CDDHR99} implemented $(n+1, \lfloor n/3 \rfloor)$-perfectly secure VSS schemes. These constructions suffice for all the applications in the current paper.
 % It is a two-stage secret sharing protocol for implementing the following functionality. In the first stage, denoted by $\VSS_\Share$, a special player referred to as dealer, shares a secret $s$ among $n$ players, in the presence of at most $t$ corrupted players. In the second stage, denoted by $\VSS_\Recon$, players exchange their views of the Share Stage and reconstruct the values. The functionality ensures that when the dealer is honest, before the second stage begins, the $t$ corrupted players have no information about the secret. Moreover, when the dealer is dishonest, at the end of the Share Stage the honest players would have realized it through an accusation mechanism that disqualifies the dealer.
\begin{definition}[Verifiable Secret Sharing]\label{def:VSS}
An $(n + 1, t)$-perfectly secure VSS scheme $\Prot_\VSS$ consists of a pair of protocols $(\VSS_\Share, \VSS_\Recon)$ that implement respectively the sharing and reconstruction phases as follows.
\begin{itemize}
\item {\bf Sharing Phase $\VSS_\Share$:} 
Player $P_{n+1}$ (referred to as dealer) runs on input a secret $s$ and randomness $r_{n+1}$, while any other player $P_i$ $(i \in [n])$ runs on input a randomness $r_i$. During this phase players can send (both
private and broadcast) messages in multiple rounds.
\item {\bf Reconstruction Phase $\VSS_\Recon$:}
Each shareholder sends its view $v_i$ $(i \in [n])$ of the Sharing Phase to each other player, and on input the views of all players (that can include bad or empty views) each player outputs a reconstruction of the secret $s$.
\end{itemize}
All computations performed by honest players are efficient. The computationally unbounded adversary can corrupt up to t players that can deviate from the above procedures. The following security properties
hold.
\begin{enumerate}
\item {\bf Perfectly Verifiable-Committing:} \label[Property]{item:def:VSS:vc}
if the dealer is dishonest, then one of the following two cases happen (i.e., with probability 1): 
\begin{enumerate}
\item \label[Case]{item:def:VSS:vc:case:1}
During the Sharing Phase, honest players disqualify the dealer, therefore they output a special value $\bot$ and will refuse to play the reconstruction phase; 
\item \label[Case]{item:def:VSS:vc:case:2}
During the Sharing Phase, honest players do not disqualify the dealer. Therefore such a phase determines a unique value $s^*$
that belongs to the set of possible legal values that does not include $\bot$, which will be reconstructed by the honest players during the
reconstruction phase.
\end{enumerate} 
\item \label[Property]{item:def:VSS:secrecy}
{\bf Secrecy:} 
if the dealer is honest, then the adversary obtains no information about the shared secret before running the protocol $\Recon$. More accurately, there exists a PPT oracle machine $\Sim^{(\cdot)}$ such that for any message $m$, and every (potentially inefficient) adversary $\Adv$ corrupting a set $T$ of parties with $|T|\le t$ during the Sharing Phase $\VSS_\Share(m)$ (denote $\Adv$'s view in this execution as $\View_{\Adv, T}(1^\secpar, m)$), the following holds: 
$\Set{\View_{\Adv, T}(1^\secpar, m)} \idind \Set{\Sim^\Adv(1^\secpar, T)}$.
 
%  and any (potentially unbounded) adversary $\Adv$


% denoted the set of corrupted parties by $A$ and their corresponding views during the sharing phase as $\Set{\view_i}_{i\in A}$. Then, for any message $m$, there exists a complementary set of view $\Set{\view_j}_{j \in [n]\setminus A}$ such that $\VSS_\Recon(\view_1, \ldots, \view_n) = m$. (Actually, given arbitrary $m$ and $\Set{\view_i}_{i\in A}$ $(|A|<t)$, the scheme from \cite{STOC:BenGolWig88,EC:CDDHR99} allows efficient construction of the set $\Set{\view_j}_{j \in [n]\setminus A}$.)

\item {\bf Correctness:}
 if the dealer is honest throughout the protocols, then each honest player will output the shared secret $s$ at the end of protocol $\Recon$.
\end{enumerate}
\end{definition}


\subsection{Information-Theoretic MPC and the MPC-in-the-Head Paradigm}
\label{add-prelim:mpc_in_the_head}
We first recall {\em information-theoretically secure} MPCs and relevant notion that will be employed in the MPC-in-the-head paradigm shown later.

\para{Information-Theoretic MPC.} We now define MPC in the information-theoretic setting (i.e., secure against unbounded adversaries). 
%Both the ideal and real executions are identical to the ones described in \Cref{sec:prelim:computational-MPC}, except that the machines $\Adv$ and $\Sim$ are computationally unbounded now.

 % Secure multi-party computation protocols allow several parties to compute a function $f$ on their joint private inputs even in the presence of corrupted parties that try to glean other parties' inputs. Formally, we consider $n$ different parties, of whom $t$ parties are corrupted. Further, let \Adv denote a real world adversary for protocol $\Prot$ that recieves auxillary input $z$, and $S$ denote an ideal world adversary for $\Prot$. Denote by $\REAL_{\Prot,\Adv(z),I}(\vec{x})$ the random variable consisting of the output of \Adv controlling a set of corrupted parties $I$, and the outputs of the honest parties with respect to an execution of $\Prot$ where party $P_i$ has input $x_i$ for $i \in [n]$, and $\vec{x} = (x_1,\dots x_n)$. Similarly, denote by $\IDEAL_{f,S(z),I}(\vec{x})$ the corresponding output of $S$ and other honest parties after an ideal execution with a trusted party computing $f$ on inputs $\vec{x}$. We refer the reader to \cite{Goldreich04} for a detailed description of the ideal and real executions.   

\begin{definition}[Perfectly/Statistically-Secure MPC]\label{def:MPC}
Let $f:(\Set{0,1}^*)^n \mapsto (\Set{0,1}^*)^n$ be an n-ary functionality, and let $\Prot$ be a protocol. We say that $\Prot$ {\em $(n,t)$-perfectly (resp., statistically) securely} computes $f$ if for every static, malicious, and (possibly-inefficient) probabilistic adversary $\Adv$ in the real model, there exists a probabilistic adversary $\Sim$ of comparable complexity (i.e., with running time polynomial in that of $\Adv$) in the ideal model, such that for every $I \subset [n]$ of cardinality at most $t$, every $\vec{x} = (x_1,\dots,x_n) \in (\Set{0,1}^*)^n$ (where $|x_1|=\dots=|x_n|$), and every $z \in \Set{0,1}^*$, it holds that: 
$$\Set{\REAL_{\Prot,\Adv(z),I}(\vec{x})} \idind \Set{\IDEAL_{f,\Sim(z),I}(\vec{x})} ~~~~\big(\text{resp.,}~\Set{\REAL_{\Prot,\Adv(z),I}(\vec{x})} \sind \Set{\IDEAL_{f,\Sim(z),I}(\vec{x})}\big).$$   
\end{definition}
%[\rohit{def from \cite{FOCS:GLOV12}}]
Recall that the MPC protocol from \cite{STOC:BenGolWig88} achieves $(n,t)$-perfect security (against static and malicious adversaries) with $t$ being a constant fraction of $n$.
\begin{theorem}[\cite{STOC:BenGolWig88}]\label{thm:BGW88}
Consider a synchronous network  with  pairwise  private  channels. Then,  for every $n$-ary functionality $f$, there exists a protocol that $(n,t)$-perfectly securely computes $f$ in the presence of a static malicious adversary for any $t < n/3$.
\end{theorem}

\para{Consistency, Privacy, and Robustness.} We now define some {notation} related to MPC protocols. Their roles will become clear when we discuss the MPC-in-the-head technique later. 
\begin{definition}[View Consistency]
\label{def:view-consistency}
A view $\View_i$ of an honest player $P_i$ during an MPC computation $\Prot$ contains input and randomness used in the computation, and all messages received from and sent to the communication tapes. A pair of views $(\View_i,\View_j)$ is {\em consistent} with each other if 
\begin{enumerate}
  \item Both corresponding players $P_i$ and $P_j$ individually computed each outgoing message honestly by using the random tapes, inputs and incoming messages specified in $\View_i$ and $\View_j$ respectively, and:
  \item All output messages of $P_i$ to $P_j$ appearing in $\View_i$ are consistent with incoming messages of $P_j$ received from $P_i$ appearing in $\View_j$ (and vice versa).  
\end{enumerate}   
\end{definition}
%[\rohit{Last two defs from \cite{FOCS:GLOV12}}]
We further define the notions of correctness, privacy and robustness for multiparty protocols. 

\begin{definition}[Semi-Honest Computational Privacy]\label{def:t-privacy}
Let $1\leq t<n$, let $\Prot$ be an MPC protocol, and let $\Adv$ be any {\em static, PPT, and semi-honest} adversary. We say that $\Prot$ realizes a function $f:(\Set{0,1}^*)^n \mapsto (\Set{0,1}^*)^n$ with {\em semi-honest $(n,t)$-computational privacy} if there is a PPT simulator $\Sim$ such that for any inputs $x,w_1,\dots,w_n$, every subset $T \subset [n]$ $(|T| \leq t)$ of players corrupted by $\Adv$, and every $D$ with circuit size at most $\mathsf{poly(\SecPar)}$, it holds that 
{\fontsize{10.5pt}{0pt}\selectfont
\begin{equation}
\big|\Pr[D(\View_T(x,w_1,\dots,w_n)) =1]- \Pr[D(\Sim(T,x,\Set{w_i}_{i \in T},f_T(x,w_1,\dots,w_n)))=1]\big| \leq \negl(\SecPar),
\end{equation}}
where $\View_T(x,w_1,\dots,w_n)$ is the joint view of all players.
% the joint view $\View_T(x,w_1,\dots,w_n)$ of players in $T$ is distributed identically to $\Sim(T,x,(wi_i)_{i \in T},f_T(x,w_1,\dots,w_n))$. The relaxations to statistical or computational privacy are defined in the natural way. That is, in the statistical (resp., computational) case we require that for every distinguisher $D$ (resp. $D$ with circuit size at most $\mathsf{poly(\SecPar)}$) there is a negligible function $\delta(\cdot)$ such that 
% \begin{equation}
% \big|\Pr[D(\View_T(x,w_1,\dots,w_n)) =1]- \Pr[D(\Sim(T,x,\Set{w_i}_{i \in T},f_T(x,w_1,\dots,w_n)))=1]\big| \leq \delta(\SecPar).
% \end{equation}
\end{definition} 


\begin{definition}[Statistical/Perfect Correctness]\label{def:MPC-correctness}
Let $\Prot$ be an MPC protocol. We say that $\Prot$ realizes a deterministic n-party functionality $f(x,w_1,\dots,w_n)$ with {\em perfect (resp., statistical)} correctness if for all inputs $x,w_1,\dots,w_n$, the probability that the output of some party is different from the output of some party is different from the actual output of $f$ is 0 (resp., negligible in $k$), where the probability is over the independent choices of the random inputs $r_1,\dots,r_n$ of these parties.   
\end{definition}



\begin{definition}[Perfect/Statistical Robustness] \label{def:t-robustness}
Assume the same setting as the previous definition. We say that $\Prot$ realizes $f$ with {\em $(n,t)$-perfect (resp., statistical) robustness} if in addition to being perfectly (resp., statistical) correct in the presence of a semi-honest adversary as above, it enjoys the following {\em robustness} property against any computationally unbounded malicious adversary corrupting a set $T$ of at most $t$ parties, and for any inputs $(x,w_1,\dots,w_n)$: if there is no $(w_1',\dots,w_n')$ such that $f(x,w_1',\dots,w_n')=1$, then the probability that some uncorrupted player outputs 1 in an execution of $\Prot$ in which the inputs of the honest parties are consistent with $(x,w_1,\dots,w_n)$ is 0 (resp., negligible in \SecPar).    
\end{definition}


\para{MPC-in-the-Head.} MPC-in-the-head is a technique developed for constructing  black-box ZK protocols from MPC protocols \cite{STOC:IKOS07}. Very roughly, the MPC-in-the-head idea is the following.  Let $\Func_\textsc{zk}$ be the zero-knowledge functionality for an \NP language. $\Func_\textsc{zk}$ takes as public input $x$ and one share from each party, and outputs 1 iff the secret reconstructed from the shares is a valid witness.
To build a ZK protocol, the prover runs in his head an execution of MPC w.r.t.\ $\Func_\textsc{zk}$ among $n$ imaginary parties, each one participating in the protocol with a share of the witness. Then, it commits to the view of each party separately. The verifier obtains $t$ randomly chosen views, checks that such views are ``consistent'' (see \Cref{def:view-consistency}), and accepts if the output of every party is 1. The idea is that, by selecting the $t$ views at random, $V$ will catch inconsistent views if the prover cheats.

We emphasize that, in this paradigm, a malicious prover decides the randomness of each virtual party, including those not checked by the verifier (corresponding to honest parties in the MPC execution). Therefore, MPC protocols with standard computational security may not protect against such attacks. We need to ensure that the adversary cannot force a wrong output even if it additionally controls the honest parties' random tapes. The $(n,\lfloor n/3 \rfloor)$-perfectly secure MPC protocol in \Cref{thm:BGW88} suffices for this purpose (see also \Cref{rmk:exact-mpc-requriements:mpc-in-the-head}).

One can extend this technique further (as in \cite{FOCS:GLOV12}), to prove a general predicate $\phi$ about an arbitrary value $\alpha$.  Namely, one can consider the functionality $\Func_\phi$ in which party $i$ participates with input a VSS share $[\alpha]_i$. $\Func_\phi$ collects all such shares, and outputs 1 iff $\phi(\VSS_\Recon([\alpha]_1,\ldots,[\alpha]_n)) = 1$.



\begin{remark}[Exact Security Requirements on the Underlying MPC.] 
\label{rmk:exact-mpc-requriements:mpc-in-the-head}
To be more accurate, any MPC protocol that achieves {\em semi-honest $(n,t)$-computational privacy (as per \Cref{def:t-privacy}) and $(n,t)$-perfect robustness (as per \Cref{def:t-robustness})} will suffice for the MPC-in-the-head application.\footnote{It is also worth noting that the $(n,t)$-perfect robustness could be replaced with {\em adaptive $(n,t)$-statistical robustness}. See \cite[Section 4.2]{STOC:IKOS07} for more details.} These two requirements are satisfied by any $(n,t)$-perfectly secure MPC (and, in particular, the one from \Cref{thm:BGW88}).
\end{remark}

==> sections/define-eps-simulatability.tex <==
%!TEX root=../main.tex
\section{Defining $\epsilon$-Simulatable Security}

==> sections/fully-PQ-2PC.tex <==
%!TEX root=../main.tex

\section{Black-Box PQ-2PC in Polynomial Rounds}
\xiao{[Check with Takashi:] what is the state-of-the-art for this topic? We need to compare with them.}

\xiao{[Check with Takashi:] We need an injective trapdoor function whose range supports oblivious sampling. Do we have constructions from lattice assumptions?}

==> sections/takashi_backup.tex <==
What is non-trivial is to prove the weak $\epsilon$-simulation-extractability.
For proving this, we prepare three lemmas. 

The first lemma claims that $\wExtCom$ satisfies extractability \emph{without simulation} of a malicious sender's internal state.
For stating the lemma, we define \emph{validness} for commitments generated in the first round of the commitment phase for convenience.
\begin{definition}\label{lem:valid-com}
We say that $\{\com_i^0,\com_i^1\}_{i=1}^{k}$ are  valid commitments for $m \in \bit^\ell$ if $\com_{i}^{b}$ is a valid commitment of $v_{i}^{b}\in \bit^\ell$ under $\Com$ for $i\in [k],b\in \bit$  and   $m=v_{i}^{0}\oplus v_{i}^{1}$ for all $i\in [k]$.
\end{definition}

\begin{lemma}\label{lem:extraction-without-simulation}
Let $\{\com_i^0,\com_i^1\}_{i=1}^{k}$ be valid commitments for $m \in \bit^\ell$, and $v_{i}^{b}$ be the committed value in $\com_i^{b}$. 
There exists a QPT algorithm $\ext_{\simless}$ such that for any quantum algorithm $\A_{\open}$ with quantum advice $\rho_\open$, if we have 
\begin{align*}
    \Pr_{\Vect{c}\sample \bit^k}[\A_{\open}(\rho_\open,\Vect{c})=\{v_{i}^{c_i}\}_{i=1}^{k}]\geq \gamma,
\end{align*}
then we have 
\begin{align*}
    \Pr[\ext_{\simless}(\{\com_i^0,\com_i^1\}_{i=1}^{k},\A_{\open},\rho_\open)=m]\geq \gamma^3- 2^{-k}.
\end{align*}
\takashi{Actually, the RHS can be improved to $\gamma(\gamma^2 - 2^{-k})$ \cite[Lemma 8]{EC:Unruh12} though this is not needed for our purpose.}
\end{lemma}
\begin{proof}[Proof of \Cref{lem:extraction-without-simulation}]
This is a straightforward application of Unruh's rewinding lemma \cite[Lemma 7]{EC:Unruh12}:
\begin{lemma}\label{lem:Unruh_rewinding}
Let $C$ be a set whose  size is denoted by $|C|$. 
Let $\{\Pi_{i}\}_{i\in C}$ be orthogonal projectors on a Hilbert space $\hil$.
Let $\ket{\phi}\in \hil$ be a unit vector. 
Let $V\defeq \sum_{i\in C}\frac{1}{|C|}\|\Pi_i\ket{\phi}\|^2$ and $F\defeq \sum_{i,j\in C}\frac{1}{|C|^2}\|\Pi_i\Pi_j\ket{\phi}\|^2$ Then we have $F\geq V^3$. 
\end{lemma}   
\end{proof}


The second is a variant of the extraction lemma 
 of \cite[Lemma 4.2]{chia2020black}.
\begin{lemma}[Extraction Lemma]\label{lem:extraction-variant} 
Let $\A$ be a QPT algorithm  that takes  a quantum input $\ket{\psi}\in \hil$ and outputs a  classical string $s$ or $\bot$.
Suppose that there exists $s^*$ such that for any $\ket{\psi}\in \hil$, $\A(\ket{\psi})$ outputs $s^*$
whenever $\A$ does not output $\bot$. 
For any noticeable $\delta$, 
there exists an orthogonal decomposition of  $\hil$ into $S_{<\delta}$ and $S_{\geq \delta}$ that satisfies the following.
\begin{enumerate}
    \item \label{item:extraction-variant:prob}
    For any normalized state $\ket{\psi_{<\delta}}\in S_{<\delta}$, it holds that $\Pr[\A(\ket{\psi_{<\delta}})=s^*]< \delta$. Similarly,  for any normalized state $\ket{\psi_{\geq \delta}}\in S_{\geq \delta}$, it holds that $\Pr[\A(\ket{\psi_{\geq \delta}})=s^*]\geq \delta$. 
    \item 
    There exists a QPT algorithm $\ext_{\CCY}$
    %, which takes a quantum input $\ket{\psi}\in \hil$ and outputs a classical string $s$ and a state $\ket{\psi'}\in \hil$, 
    that satisfies the following.  
    \begin{enumerate}
        \item \label{item:extraction-variant:extraction}
        For any normalized state $\ket{\psi_{\geq \delta}}\in S_{\geq \delta}$, it holds that 
        \begin{align*}
        \Pr[s=s^*\land \|\ket{\psi_{\geq \delta}}\bra{\psi_{\geq \delta}}-\ket{\psi'_{\geq \delta}}\bra{\psi'_{\geq \delta}}\|_{tr}=\negl(\secpar) :(s,\ket{\psi'_{\geq \delta}})\sample \ext_{\CCY}(1^{\delta^{-1}},\A_{\CCY}, \ket{\psi_{\geq \delta}})]=1-\negl(\secpar)
        \end{align*}
        where the probability is over intermediate measurement results by $\ext_\CCY$.\footnote{Usually, we consider an output of a quantum algorithm as a mixed state taking all the randomness into account. On the other hand, here we consider the output of $\ext_\CCY$ as a probabilistic variable that takes pure states.}\takashi{I'm not sure if this explanation makes sense.}
        \item \label{item:extraction-variant:invariant}
        For any normalized state $\ket{\psi_{< \delta}}\in S_{< \delta}$, 
        \begin{align*}
        \Pr[\ket{\psi'_{< \delta}}\in S_{<\delta }:(s,\ket{\psi'_{< \delta}})\sample \ext_{\CCY}(1^{\delta^{-1}},\A_{\CCY}, \ket{\psi_{\geq \delta}})]=1
        \end{align*}
    where the probability is over intermediate measurement results by $\ext_\CCY$.
    \end{enumerate} 
\end{enumerate}
\begin{comment}
Let $\A$ be a QPT algorithm  that takes  a quantum input $\inp$ and outputs a  classical string $s$ or $\bot$.
Suppose that there exists $s^*$ such that for any input $\inp$, $\A(\inp)$ outputs $s^*$
whenever $\A$ does not output $\bot$. 
Let $\B$ be a QPT algorithm that takes a quantum input $\rho$ (in the same space as that of $\A$) and outputs a bit $b$.
Suppose that there is a constant $c$ such that for any input $\rho$,  
    $Pr[\B(\inp)=1]\leq (\Pr[\A(\inp)\neq \bot])^c$.
There there exists a QPT algorithm  $\ext_\CCY$, which takes $\inp$ as input and outputs a classical string $s_\ext$ and a quantum state $\rho_\ext$, satisfying the following.  
For any noticeable $\epsilon$,  we define the following two experiments. 
\begin{tabular}{l|l}
    \begin{minipage}[t]{0.50\textwidth}
\underline{$\Exp_{\mathsf{real}}[\B](\secpar,\inp)$}\\
~\vspace{1mm}\\
$b\sample \B(\inp)$,\\
\emph{If} $b= 1$,\\
$~~~~$\emph{Output} $\bot$\\
\emph{Else Output} $(s,\out)$.
    \end{minipage} 
        &~
    \begin{minipage}[t]{0.50\textwidth}
\underline{$\Exp_{\mathsf{ext}}[\A,\ext_\CCY](\secpar,\epsilon,\inp)$}\\
$(m_\ext,\inp_\ext)\sample \ext_\CCY(\inp)$\\
$(b,s,\out)\sample \A(\inp_\ext)$,\\
\emph{If} $b\neq 1$,\\
$~~~~$\emph{Output} $\bot$\\
\emph{Else Output} $(s,\out)$.
    \end{minipage} 
    \end{tabular}\\

There exists a QPT extractor $\Ext_\CCY$ of the above form such that for any $\A$ of the above form, $\A$'s input $\inp$, and a noticeable $\epsilon$, we have 
\begin{align*}
    \{\Exp_{\mathsf{real}}[\A](\secpar,\inp)\}_{\secpar\in \mathbb{N}}\statind_\epsilon \{\Exp_{\mathsf{ext}}[\A,\ext_\CCY](\secpar,\epsilon,\inp)\}_{\secpar\in \mathbb{N}}.
\end{align*}
\end{comment}
\end{lemma}
%\begin{remark}
%This is a generalized version of the 
%\emph{statistically binding} case of the  extraction lemma of \cite{chia2020black}. 
%The extraction lemma of \cite{chia2020black} is also shown to hold for the strong collapse-binding case, which is incomparable to \Cref{lem:extraction-variant}.
%\end{remark}
\begin{proof}[Proof of \Cref{lem:extraction-variant}]
This is implicitly proven in  \cite{chia2020black}. 
Roughly, Jordan's lemma naturally gives such a decomposition. 
%, which in turn is based on Jordan's lemma.
%Actually,  the proof is even simpler than theirs because we consider a simpler  abstracted setting. (Essentially, we only need to prove \cite[Claim4.5]{chia2020black}.)
\takashi{We may add the proof in Appendix later for which we can recycle many materials from \cite{chia2020black}.}
\end{proof}

The third is a simple technical lemma  that is obtained by generalizing the analysis in   \cite{chia2020black}. 
\begin{lemma}\label{lem:state-close}
Let $\ket{\phi_b}=\ket{\phi_{b,0}}+\ket{\phi_{b,1}}$ be a (not necessarily normalized) state such that $\bra{\phi_{b,0}}\ket{\phi_{b,1}}=0$
for $b\in \bit$.
%such that $\|\ket{\phi_{0,1}}-\ket{\phi_{1,1}}\|\leq \eta$.
Let $F$ be a quantum algorithm  such that 
$\Pr[F(\ket{\phi_{b,0}})=\bot]\geq 1-\gamma$ for $b\in \bit$ where $\gamma< 1/729$.  
%where $u$ is a classical string, $p_b\leq \gamma$ 
%for $b\in \bit$.  
%there exists a classical string $u$ such that 
%$\Pr[M\circ F(\phi_b)=u]=1-\gamma$ where $M\circ F(\phi_b)$ denotes the measurement of $F(\phi_b)$ in the computational basis. 
Then for any distinguisher $D$, it holds that 
\begin{align*}
    |\Pr[D(F(\ket{\phi_0}\bra{\phi_0}))=1]
    -\Pr[D(F(\ket{\phi_1}\bra{\phi_1}))=1]|\leq 6\gamma^{1/6} +
    %\TD(\ket{\phi_{0,1}},\ket{\phi_{1,1}}).
    \|\ket{\phi_{1,1}}\bra{\phi_{1,1}}-\ket{\phi_{0,1}}\bra{\phi_{0,1}}\|_{tr}.
\end{align*}
%\begin{align*}
%    \|F(\ket{\phi_0}\bra{\phi_0})-F(\ket{\phi_1}\bra{\phi_1}))\|_{tr}\leq \gamma + \|\ket{\phi_{0,1}}\bra{\phi_{0,1}}-\ket{\phi_{1,1}}\bra{\phi_{1,1}}\|_{tr}.
%\end{align*}
\takashi{The current proof is based on CCY21. I believe this is correct, but very awkward. 
Especially, I don't find any essential reason why the loss of $6$-th power occurs. Can we find an easier proof possibly with a better bound?
(Additional note: In CCY21, the loss was cubic. This difference comes from the fact that we do not assume that $F$ is closed under Jordan's subspace for generality.
This impacts the RHS of \Cref{item:bound_probability} of \Cref{cla:useful_properties}.
The additional term could be $\gamma$ in CCY21.)
}
\end{lemma}
\begin{proof}
Let 
$\ket{\phi'_1}=\ket{\phi_{1,0}}+\ket{\phi_{0,1}}$.
It is easy to see that 
\begin{align*}
    \|\ket{\phi_1}\bra{\phi_1}-\ket{\phi'_1}\bra{\phi'_1}\|_{tr}
    \leq \|\ket{\phi_{1,1}}\bra{\phi_{1,1}}-\ket{\phi_{0,1}}\bra{\phi_{0,1}}\|_{tr}.
\end{align*}
\begin{takashienv}{}
Is there any obvious explanation why the above holds? I thought this holds by the following:
\begin{align*}
    \|\ket{\phi_1}\bra{\phi_1}-\ket{\phi'_1}\bra{\phi'_1}\|_{tr}
    &=\|\ket{\phi_{1,0}}(\bra{\phi_{1,1}}-\bra{\phi_{0,1}})+(\ket{\phi_{1,1}}-\ket{\phi_{0,1}})\bra{\phi_{1,0}}+\ket{\phi_{1,1}}\bra{\phi_{1,1}}-\ket{\phi_{0,1}}\bra{\phi_{0,1}}\|_{tr}\\
    &\leq \|\ket{\phi_{1,0}}(\bra{\phi_{1,1}}-\bra{\phi_{0,1}})+(\ket{\phi_{1,1}}-\ket{\phi_{0,1}})\bra{\phi_{1,0}}\|_{tr}
    +\|\ket{\phi_{1,1}}\bra{\phi_{1,1}}-\ket{\phi_{0,1}}\bra{\phi_{0,1}}\|_{tr}\\
\end{align*}
and 
\begin{align*}
    \|\ket{\phi_{1,0}}(\bra{\phi_{1,1}}-\bra{\phi_{0,1}})+(\ket{\phi_{1,1}}-\ket{\phi_{0,1}})\bra{\phi_{1,0}}\|_{tr}=0
\end{align*}
because this operator is isomorphic to the Pauli $X$ in the 2-dimensional space spanned by $\ket{\phi_{1,0}}$ and $\ket{\phi_{1,1}}-\ket{\phi_{0,1}}$. 
\end{takashienv}
Therefore, it suffices to show that for any distinguisher $D$, it holds that 
\begin{align*}
    \left|\Pr[D(F(\ket{\phi_0}\bra{\phi_0}))=1]
    -\Pr[D(F(\ket{\phi_1}\bra{\phi_1}))=1]\right|\leq 6\gamma^{1/6}
\end{align*}
assuming that $\ket{\phi_{0,1}}=\ket{\phi_{1,1}}$. 

$F$ can be represented by a projector $\Pi$ over the input register and auxiliary input register with which $F$ works as follows.
$F$ appends the ancillary register initialized to $\ket{0^n}$, performs the measurement $\{\Pi,I-\Pi\}$ on the input and ancillary registers, and outputs the state in a designated output register tracing out all other registers if $\Pi$ is applied, and otherwise outputs $\bot$.
Since tracing out registers only make the task of distinguisher more difficult, we only have to prove 
\begin{align}
\label{eq:conclusion_trace_distance}
   \|\rho_0-\rho_1\|_{tr}\leq  6\gamma^{1/6}
\end{align}
where 
\begin{align*}
\rho_{b}\defeq (1-p_b)\ket{\bot}\ket{\bot}\bra{\bot}\bra{\bot}+\Pi\ket{\phi_b}\ket{0^n}\bra{\phi_b}\bra{0^n}\Pi,
\end{align*}
%\begin{align*}
%\hat{\rho}\defeq (1-\hat{p})\ket{\bot}\bra{\bot}+\Pi\hat{\ket{\psi}}\ket{0^n}\hat{\bra{\psi}}\bra{0^n}\Pi 
%\end{align*}
for
\begin{align*}
p_b \defeq \|\Pi\ket{\phi_b}\ket{0^n}\|^2.
\end{align*}

Here, we show the following claim.
\begin{myclaim}\label{cla:useful_properties}
The following holds:
\begin{enumerate}
    \item \label{item:norm_of_projected_state} 
    $\|\Pi\ket{\phi_{b,0}\ket{0^n}}\|^2\leq \gamma$ for $b\in \bit$.
    \item \label{item:bound_probability}
    $\|\Pi\ket{\phi_{b,1}}\ket{0^n}\|^2\leq p_b\leq  \|\Pi\ket{\phi_{b,1}}\ket{0^n}\|^2+3\gamma^{1/2}$
    for $b\in \bit$.
\end{enumerate}
\end{myclaim}
\begin{proof}[Proof of \Cref{cla:useful_properties}]
\Cref{item:norm_of_projected_state} directly follows from the definition of $\Pi$ and the assumption that $\Pr[F(\ket{\phi_{b,0}})=\bot]\geq 1-\gamma$. 
The first inequality of \Cref{item:bound_probability} clearly follows from the definition of $p_b$ and $\ket{\phi_b}=\ket{\phi_{b,0}}+\ket{\phi_{b,1}}$. 
The second inequality of \Cref{item:bound_probability} can be shown as follows:
\begin{align*}
    p_b&=\|\Pi\ket{\phi_b}\ket{0^n}\|^2\\
    &=\|\Pi\ket{\phi_{b,0}}\ket{0^n}+\Pi\ket{\phi_{b,1}}\ket{0^n}\|^2\\
    &\leq \|\Pi\ket{\phi_{b,0}}\ket{0^n}\|^2+\|\Pi\ket{\phi_{b,1}}\ket{0^n}\|^2 
    + 2\|\Pi\ket{\phi_{b,0}}\|\cdot \|\Pi\ket{\phi_{b,1}}\|\\
    %+ 2|\ipro{\phi_{b,0}}{\phi_{b,1}}|\\
    &\leq \|\Pi\ket{\phi_{b,1}}\ket{0^n}\|^2+ 3\gamma^{1/2}
\end{align*}
where the last inequality follows from $\|\Pi\ket{\phi_{b,0}}\ket{0^n}\|^2\leq \|\Pi\ket{\phi_{b,0}}\ket{0^n}\|\leq \gamma^{1/2}$ by \Cref{item:norm_of_projected_state} and
$\|\Pi\ket{\phi_{b,1}}\|\leq 1$. 
\end{proof}



The rest of the proof is very similar to (the latter half of) that of \cite[Claim 4.5]{chia2020black}. 
We apply  
\cite[Lemma 3.1]{chia2020black}
%\ref{lem:bound_trace_distance} 
by setting
\begin{align*} 
&\ket{\psi_0}:=\frac{\Pi\ket{\phi_0}\ket{0^n}}{\|\Pi\ket{\phi_0}\ket{0^n}\|}=p_0^{-1/2}\Pi\ket{\phi_0}\ket{0^n},\\
&\ket{\psi_1}:= \frac{\Pi\ket{\phi_1}\ket{0^n}}{\|\Pi\ket{\phi_1}\ket{0^n}\|}=p_1^{-1/2}\Pi\ket{\phi_1}\ket{0^n},\\
&\ket{\psi'_0}=\ket{\psi'_1}:
=\ket{\bot}\ket{\bot},\\
&\tilde{p}\defeq \|\Pi\ket{\phi_{0,1}}\ket{0^n}\|^2=\|\Pi\ket{\phi_{1,1}}\ket{0^n}\|^2.\footnote{Recall that we are assuming $\ket{\phi_{0,1}}=\ket{\phi_{1,1}}$.}
\end{align*}
Then we have
\begin{align}
\|\rho_0-\rho_1\|_{tr}\leq |p_0-\tilde{p}|+ |p_1-\tilde{p}|+ \tilde{p}\sqrt{1-|\ipro{\psi_0}{\psi_1}|^2}.
\label{eq:bound_trace_distance_expand} 
\end{align}

We give an upper bound for each term.\\
\noindent\textbf{Upper bound of $|p_b-\tilde{p}|$.}
\Cref{item:bound_probability} of \Cref{cla:useful_properties} directly gives  
\begin{align}
|p_b-\tilde{p}|\leq 3\gamma^{1/2}.  \label{eq:bound_first_and_second_term}
\end{align}

\noindent\textbf{Upper bound of $\tilde{p}\sqrt{1-|\ipro{\psi_0}{\psi_1}|^2}$.}
If we have $\tilde{p}\leq \gamma^{1/6}$, then there is a trivial upper bound by $\gamma^{1/6}$.
We assume $\tilde{p}>\gamma^{1/6}$ in the following.
For giving an upper bound of $\tilde{p}\sqrt{1-|\ipro{\psi_0}{\psi_1}|^2}$, we give a lower bound of $|\ipro{\psi_0}{\psi_1}|$.
By the definitions  of $\ket{\psi_0}$ and $\ket{\psi_1}$, we have 
\begin{align}
|\ipro{\psi_0}{\psi_1}|&=p_0^{-1/2}\cdot p_1^{-1/2}\cdot
\left|
\begin{array}{cc}
\bra{\phi_{0,0}}\bra{0^n}\Pi\ket{\phi_{1,0}}\ket{0^n}&+
\bra{\phi_{0,0}}\bra{0^n}\Pi\ket{\phi_{1,1}}\ket{0^n}\\
+\bra{\phi_{0,1}}\bra{0^n}\Pi\ket{\phi_{1,0}}\ket{0^n}
&+\bra{\phi_{0,1}}\bra{0^n}\Pi\ket{\phi_{1,1}}\ket{0^n}
\end{array}
\right| \notag \\
\begin{split}
&\geq p_0^{-1/2}\cdot p_1^{-1/2}\cdot\left|\bra{\phi_{0,1}}\bra{0^n}\Pi\ket{\phi_{1,1}}\ket{0^n}\right|- p_0^{-1/2}\cdot p_1^{-1/2}\cdot\left|\bra{\phi_{0,0}}\bra{0^n}\Pi\ket{\phi_{1,0}}\ket{0^n}\right|\\
&~~~-p_0^{-1/2}\cdot p_1^{-1/2}\cdot\left|\bra{\phi_{0,0}}\bra{0^n}\Pi\ket{\phi_{1,1}}\ket{0^n}\right|
-p_0^{-1/2}\cdot p_1^{-1/2}\cdot\left|\bra{\phi_{0,1}}\bra{0^n}\Pi\ket{\phi_{1,0}}\ket{0^n}\right|.
\end{split}
\label{eq:lower_bound_ipro}
\end{align}
In the following, we give bounds for each term of \Cref{eq:lower_bound_ipro}.  


The first term is bounded as follows:
\begin{align}
&p_0^{-1/2}\cdot p_1^{-1/2}\cdot\left|\bra{\phi_{0,1}}\bra{0^n}\Pi\ket{\phi_{1,1}}\ket{0^n}\right| \notag \\
= &p_0^{-1/2}\cdot p_1^{-1/2}\cdot \|\Pi\ket{\phi_{0,1}}\ket{0^n}\|\cdot \|\Pi\ket{\phi_{1,1}}\ket{0^n}\| \notag\\
\geq &\frac{\|\Pi\ket{\phi_{0,1}}\ket{0^n}\|}{\sqrt{\|\Pi\ket{\phi_{0,1}}\ket{0^n}\|^2+3\gamma^{1/2}}}\cdot \frac{\|\Pi\ket{\phi_{1,1}}\ket{0^n}\|}{\sqrt{\|\Pi\ket{\phi_{1,1}}\ket{0^n}\|^2+3\gamma^{1/2}}} \notag\\
\geq &\left( 1- \frac{3\gamma^{1/2}}{\|\Pi\ket{\phi_{0,1}}\ket{0^n}\|^2}\right)\cdot \left( 1- \frac{3\gamma^{1/2}}{\|\Pi\ket{\phi_{1,1}}\ket{0^n}\|^2}\right) \notag\\
\geq &\left( 1- \frac{3\gamma^{1/2}}{\gamma^{1/6}}\right)\cdot \left( 1- \frac{3\gamma^{1/2}}{\gamma^{1/6}}\right) \notag\\
\geq &1- 6\gamma^{1/3}. \label{eq:lower_bound_geqt}
\end{align}
where the first equality follows from
the assumption that $\ket{\phi_{0,1}}=\ket{\phi_{1,1}}$, 
the first inequality follows from 
\Cref{item:bound_probability} of \Cref{cla:useful_properties}, 
the second inequality follows from 
the fact that we have 
$\frac{a}{\sqrt{a^2+b}}\geq 1-\frac{b}{a^2}>0$ for any reals $a,b$ such that $a^2>b>0$,\footnote{We note that we have $\|\Pi\ket{\phi_{b,1}}\ket{0^n}\|>3\gamma^{1/2}$  since we assume $\tilde{p}>\gamma^{1/6}$ and $\gamma<1/729$.}  
and the third inequality follows from the assumption that $\tilde{p}\geq \gamma^{1/6}$. 

The second, third, and fourth terms are bounded as follows.
For $(a,b)\in \{(0,0),(0,1),(1,0)\}$, we have 
\begin{align}
&p_0^{-1/2}\cdot p_1^{-1/2}\cdot\left|\bra{\phi_{0,a}}\bra{0^n}\Pi\ket{\phi_{1,b}}\ket{0^n}\right| \notag \\
\leq  &\frac{\|\Pi\ket{\phi_{0,a}}\ket{0^n}\|\cdot \|\Pi\ket{\phi_{1,b}}\ket{0^n}\|}{\|\Pi\ket{\phi_{0,1}\ket{0^n}}\cdot \Pi\ket{\phi_{1,1}}\ket{0^n}\|} \notag\\
\leq &\frac{\gamma^{1/2}}{\tilde{p}} 
\leq \gamma^{1/3} \label{eq:lower_bound_leqt}
\end{align}
where the first inequality follows from \Cref{item:bound_probability} of \Cref{cla:useful_properties}, the second inequality follow from \Cref{item:norm_of_projected_state} of \Cref{cla:useful_properties}, and the third inequality follows from the assumption that $\tilde{p}\geq \gamma^{1/6}$.

By combining Eq. \ref{eq:lower_bound_ipro}, \ref{eq:lower_bound_geqt}, and \ref{eq:lower_bound_leqt},    we have 
\[
|\ipro{\psi_0}{\psi_1}|\geq 1- 9\gamma^{1/3} >0
\]
where the latter inequality holds since we assume $\gamma<1/729$. 
Therefore we have
\begin{align}
\tilde{p}\sqrt{1-|\ipro{\psi_0}{\psi_1}|^2}
&\leq \tilde{p}\sqrt{18\gamma^{1/3} } \notag \\
&\leq 5\gamma^{1/6}.   \label{eq:bound_third_term}
\end{align} 
We note that Eq. \ref{eq:bound_third_term} also holds for the case of  $\tilde{p}\leq \gamma^{1/6}$. 
By plugging Eq. \ref{eq:bound_first_and_second_term} and \ref{eq:bound_third_term} into Eq. \ref{eq:bound_trace_distance_expand} and $6\gamma^{1/2}< \gamma^{1/6}$ by $\gamma<1/729$, we obtain  \Cref{eq:conclusion_trace_distance}. 
This completes the proof of \Cref{lem:state-close}.
\end{proof}

With \Cref{lem:extraction-without-simulation,lem:extraction-variant,lem:state-close} at hand, we are ready to prove \Cref{thm:wExtCom}.

\begin{proof}[Proof of \Cref{thm:wExtCom}]
Correctness, statistical binding, and computational hiding are almost clear.
We prove the $\epsilon$-simulation-extractability in the following.
Let $S^*$ be a QPT malicious sender with quantum advice $\rho$.  
%By considering purification, it suffices to prove the $\epsilon$-simulation when $\rho$ is a pure state.
%Therefore we assume so and denote $\rho$ by $\ket{\psi_\aux}$. 
We call 
\Cref{item:extcom:com,item:extcom:challenge} of  $S^*$  
the first and second stages of $S^*$ and denote them by $S^*_1$ and $S^*_2$, respectively. 

The weak extractor $\ext_\weak(1^\secpar,1^{\epsilon^{-1}},S^*,\rho)$  works as follows.
\begin{enumerate}
%\item 
%Prepare registers $\regaux$, 
%$\{\regCom_i^{b}\}_{i\in [k],b\in \bit}$, 
%$\{\regV_i\}_{i\in [k]}$, 
%$\regS$ and 
%initialize $\regaux$  to be $\rho$ and all other registers to be $\ket{0}$ similarly to $S^*$.  
\item 
$\ext_\weak$ runs the first stage of $S^*(1^\secpar,\rho)$, 
%i.e., 
%$U_0$ on $\regaux, \{\regCom_i^{b}\}_{i\in [k],b\in \bit}, \regS$, measure $\{\regCom_i^{b}\}_{i\in [k],b\in \bit}$
 to obtain $\vcom=\{\com_i^{0},\com_i^{1}\}_{i\in [k]}$.
Let $\rho'$ be the internal state  of $S^*$ at this point.
\item 
We apply \Cref{lem:extraction-without-simulation} where we define $\A_{\open}$ to be the second stage of $S^*$. 
%and $\rho_{\open}$ to be $\rho'$.
Let $\ext_{\simless}$ be the corresponding simulation-less extractor. 
\item 
We apply \Cref{lem:extraction-variant} where 
we define $\A_{\CCY}$ to be $\ext_{\simless}(\{\com_i^{b}\}_{i\in [k],b\in \bit},\A_{\open},\cdot)$ where $s^*$ is set to be $m_{\vcom}$. 
Let $\ext_{\CCY}$ be the corresponding extractor.
\item
$\ext_\weak$  runs $(m_\ext,\rho'')\sample \ext_{\CCY}(1^{\delta^{-1}},\A_{\CCY},\rho')$ where we set $\delta\defeq \frac{1}{216}\epsilon^{18}+2^{-k}$.  
%where all the intermediate measurements are  differed, only the output is measured, and then the computation is uncomputed.
%After the uncomputation, it measures all ancillary qubits and aborts if the measurement results are not all $0$. 
%Let $m_\ext$ be the measured output and $\rho''$ be the state in the register of $\rho'$ after the execution.
%We denote this procedure by $(m_\ext,\rho'')\sample \widetilde{\ext}_{\CCY}(1^{\delta^{-1}},\A_{\CCY},\rho')$
%Note that $\rho''$ may be different from $\rho'$ because there is a measurement before the uncomputation.  
\item $\ext_\weak$  runs 
the second stage of $S^*$ with its internal state $\rho''$ to get the decommitments $\vv,\vr$ as well as the internal state $\rho_\ext$ of $S^*$ after the execution. 
If $\vv,\vr$ is invalid opening to $\vcom$, $\ext_\weak$  aborts. 
Otherwise, it outputs $\Trans\defeq (\vcom,\vc,\vv,\vr)$, $m_\ext$, and $\inp_\ext$. 
\end{enumerate}

We show that the above extractor satisfies the requirement of the weak $\epsilon$-simulation-extractability. 
When $\vcom$ is invalid (in the sense of \Cref{lem:valid-com}), the transcript
$\Trans=(\vcom,\vc,\vv,\vr)$
is also invalid (in the sense of \Cref{def:epsilon-simext-com}).
Moreover, the distribution of $\vcom$ is the same in both the real execution and the simulation by $\ext_{\weak}$.   
Since the weak $\epsilon$-simulation-extractability requires nothing when the transcript is invalid,  it suffices to prove the weak extractor works for any fixed valid $\vcom$ and internal quantum state $\rho'$ at this point. 
That is, it suffices to prove the following lemma.
\begin{lemma}\label{lem:extraction-fixed-com}
Let $\vcom\defeq \{\com_i^{b}\}_{i\in [k],b\in \bit}$ be valid commitments with the corresponding message $m_{\vcom}$. 
For any quantum state $\rho'$, we define the following two experiments.

\begin{tabular}{l|l}
    \begin{minipage}[t]{0.50\textwidth}
\underline{$\Exp_{\mathsf{real}}^{\vcom}(\secpar,\rho')$}\\
~\vspace{1mm}\\
$\vc\sample \bit^k$\\
$(\{(v_{i},r_{i}\}_{i=1}^{k},\rho'')\sample S^*_{2}(\rho')$,\\
\emph{If} $\Com(v_{i};r_{i})\neq \com_{i}^{c_i}$\emph{for some }$i\in[k]$,\\
$~~~~$\emph{Output} $\bot$\\
\emph{Else Output} $(\vc,\{(v_{i},r_{i}\}_{i=1}^{k},m_{\vcom},\rho'')$.
    \end{minipage} 
        &~
    \begin{minipage}[t]{0.50\textwidth}
\underline{$\Exp_{\mathsf{ext}}^{\vcom}(\secpar,\rho')$}\\
$(m_\ext,\rho_\CCY)\sample \ext_{\CCY}(1^{\delta^{-1}},\A_{\CCY},\rho')$\\
$\vc\sample \bit^k$\\
$(\{(v_{i},r_{i}\}_{i=1}^{k},\rho_\ext)\sample S^*_{2}(\rho_\CCY)$,\\
\emph{If} $\Com(v_{i};r_{i})\neq \com_{i}^{c_i}$\emph{for some }$i\in[k]$,\\
$~~~~$\emph{Output} $\bot$\\
\emph{Else Output} $(\vc,\{(v_{i},r_{i}\}_{i=1}^{k},m_{\ext},\rho_\ext)$.
    \end{minipage} 
    \end{tabular}\\
Then we have 
\begin{align}\label{eq:real-ext-difference}
\{\Exp_{\mathsf{real}}^{\vcom}(\secpar,\rho')\}_{\secpar \in \mathbb{N}}\statind_{\epsilon}  
\{\Exp_{\mathsf{ext}}^{\vcom}(\secpar,\rho')\}_{\secpar \in \mathbb{N}}.
\end{align}
\end{lemma}
\begin{proof}[Proof of \Cref{lem:extraction-fixed-com}]
By purification, we can assume that $\rho'$ is a pure state 
without loss of generality, and we denote it by $\ket{\psi}$.  
Let $S_{< \delta}$ and $S_{\geq \delta}$ be as in \Cref{lem:extraction-variant}.
We decompose $\ket{\psi}$ as $\ket{\psi}=\ket{\psi_{<\delta}}+\ket{\psi_{\geq \delta}}$ where $\ket{\psi_{<\delta}}\in S_{<\delta}$ and $\ket{\psi_{\geq \delta}}\in S_{\geq \delta}$. 
By 
\Cref{item:extraction-variant:prob} of \Cref{lem:extraction-variant}, for any $\ket{\psi_{\geq \delta}}\in S_{\geq \delta}$,  
it holds that $\Pr[\A_\CCY(\ket{\psi_{\geq \delta}})=m_{\vcom}]\geq \delta$. 
Then,  
by \Cref{lem:extraction-without-simulation}, for any $\ket{\psi_{\geq \delta}}\in S_{ \geq \delta}$, it holds that 
$$\Pr[m_\ext=m_{\vcom} \land \|\ket{\psi_{\geq \delta}}\bra{\psi_{\geq \delta}}-\ket{\psi_{\CCY,\geq \delta}}\bra{\psi_{\CCY,\geq \delta}}\|_{tr}\leq \negl(\secpar):(m_\ext,\ket{\psi_{\CCY,\geq \delta}})\sample \ext_\CCY(\ket{\psi_{\geq \delta}})]=1-\negl(\secpar),$$ where the probability over the randomness of internal measurements by $\ext_\CCY$.  
On the other hand, 
by \Cref{item:extraction-variant:invariant}, for any 
$\ket{\psi_{< \delta}}\in S_{ < \delta}$, it holds that 
$$\Pr[\ket{\psi_{\CCY,<\delta}}\in S_{<\delta}:(m_\ext,\ket{\psi_{\CCY,\delta}})\sample\ext_\CCY(\ket{\psi_{< \delta}})]=1.$$ 
Combining them, 
with overwhelming probability  
the output of $\ext_{\CCY}(1^{\delta^{-1}},\A_{\CCY},\ket{\psi})$ can be written as a state 
$\ket{m'} \ket{\psi_{\CCY,<\delta}}+ \ket{m_{\vcom}}\ket{\psi_{\CCY,\geq \delta}}$
where $m'$ is some classical string, 
$\|\ket{\psi_{\geq \delta}}\bra{\psi_{\geq \delta}}-\ket{\psi_{\CCY,\geq \delta}}\bra{\psi_{\CCY,\geq \delta}}\|_{tr}\leq \negl(\secpar)$, and 
$\ket{\psi_{\CCY,<\delta}}\in S_{<\delta}$.
We apply \Cref{lem:state-close} where we set 
%$\ket{\phi_0}\defeq \ket{\psi}$,
$\ket{\phi_{0,0}}\defeq \ket{m_{\vcom}}\ket{\psi_{<\delta}}$, 
$\ket{\phi_{0,1}}\defeq \ket{m_{\vcom}}\ket{\psi_{\geq \delta}}$,
%$\ket{\phi_1}\defeq \ket{\psi}$, 
$\ket{\phi_{1,0}}\defeq \ket{m'}\ket{\psi_{\CCY,<\delta}}$,  
$\ket{\phi_{0,1}}\defeq \ket{m_{\vcom}}\ket{\psi_{\CCY, \geq \delta}}$, 
$F$ is a quantum algorithm that works as follows:
\begin{description}
\item[$F(\ket{m}\ket{\psi})$:]
It samples $\vc\sample \bit^k$, runs $(\{(v_{i},r_{i}\}_{i=1}^{k},\ket{\psi'})\sample S^*_{2}(\ket{\psi})$, and outputs $\ket{m}\ket{\vc}\ket{(v_{i},r_{i}\}_{i=1}^{k}}\ket{\psi'}$ if $\{(v_{i},r_{i}\}_{i=1}^{k}$ is a valid opening to $\{\com_i^{c_i}\}_{i=1}^{k}$ and otherwise outputs $\bot$. 
\end{description}
Then, for any distinguisher $D$, it holds that 
\begin{align*}
    &|\Pr[D(F(\ket{\phi_0}\bra{\phi_0}))=1]
    -\Pr[D(F(\ket{\phi_1}\bra{\phi_1}))=1]|\\
    &\leq 6\gamma^{1/6} +  
    \|\ket{m_{\vcom}}\ket{\psi_{\geq \delta}}\bra{m_{\vcom}}\bra{\psi_{\geq \delta}}-\ket{m_{\vcom}}\ket{\psi_{\CCY,\geq \delta}}\bra{m_{\vcom}}\bra{\psi_{\CCY,\geq \delta}}\|_{tr}.
\end{align*}
where  $\gamma\defeq   \max\{\Pr[F(\ket{\phi_{0,0}})\neq \bot],\Pr[F(\ket{\phi_{1,0}})\neq \bot]\}$ if $\gamma<1/729$. 
This means that 
\begin{align} \label{eq:real-ext-difference-two}
\{\Exp_{\mathsf{real}}^{\vcom}(\secpar,\rho')\}_{\secpar \in \mathbb{N}}\statind_{6\gamma^{1/6}}  
\{\Exp_{\mathsf{ext}}^{\vcom}(\secpar,\rho')\}_{\secpar \in \mathbb{N}}.
\end{align}
By the definitions of $F$ and $\A_{\CCY}$  and \Cref{lem:extraction-without-simulation}, for any $\ket{m}\ket{\psi}$, we have 
\begin{align*}
    \Pr[F(\ket{m}\ket{\psi})\neq \bot]\leq (\Pr[\A_{\CCY}(\ket{\psi})= s^*]+2^{-k})^{1/3}. 
\end{align*}
By \Cref{item:extraction-variant:prob} of \Cref{lem:extraction-variant}, we have 
\begin{align*}
   \Pr[\A_{\CCY}(\ket{\psi_{<\delta}})= s^*]<\delta
\end{align*}
and 
\begin{align*}
   \Pr[\A_{\CCY}(\ket{\psi_{\CCY,<\delta}})= s^*]<\delta.
\end{align*}
Combining the above, we have 
$\gamma \leq (\delta+2^{-k})^{1/3}$.  
Since we set $\delta\defeq \frac{1}{216}\epsilon^{18}-2^{-k}$, we have $6\gamma^{1/6}\leq \epsilon$
and thus $\gamma<1/729$ holds for sufficiently large security parameter $\secpar$.  
By plugging $6\gamma^{1/6}\leq \epsilon$ into \Cref{eq:real-ext-difference-two}, we get \Cref{eq:real-ext-difference}. 
This completes the proof of \Cref{lem:extraction-fixed-com}.
 \end{proof}
As already explained, \Cref{lem:extraction-fixed-com} 
implies the weak $\epsilon$-simulation-extractability, which  completes the proof of \Cref{thm:wExtCom}
\end{proof}

%We prove that $\wExtCom$ satisfies a weaker version of $\epsilon$-simulation extractability, which we call \emph{valid-commitment $\epsilon$-simulation extractability}. Roughly speaking, valid-commitment $\epsilon$-simulation extractability means that the extractor is only required to work if the commitments $\vcom=\{\com_i^0,\com_i^1\}_{i=1}^{k}$ generated in  \Cref{item:extcom:com} in the commit stage is valid. 
%For formally defining this property, we prepare the following definitions:

%\begin{definition}[Validness of $\com$]\label{def:valid_com}
%For a commitment $\com$ of the commitment scheme $\Com$, 
%we define $v_\com$ to be $v$ such that the receiver of $\Com$ accepts the message  $v$ with some opening information $r$ for $\com$ in the decommit stage if such $v$ uniquely exists, and otherwise set to be $\bot$.
%\end{definition}
\begin{definition}[Validness of $\vcom$]\label{def:valid_vcom}
For a sequence $\vcom=\{\com_{i}^{0},\com_{i}^{1}\}_{i=1}^{k}$ of commitments of the commitment scheme $\Com$, we say that $\vcom$ is valid if there exists $m\in \bit^\ell$ such that 
$v_{\com_{i}^{b}}\neq \bot$ for all $i\in[k]$ and $b\notin \bit$ and
$v_{\com_{i}^{0}}\oplus v_{\com_{i}^{1}}=m$ for all $i\in[k]$ where $v_{\com_{i}^{b}}$ is as defined in \Cref{def:valid_com}.
We denote by $m_{\vcom}$ to mean such $m$ if $\vcom$ is valid and otherwise  $\bot$. 
\end{definition}
\begin{definition}[Accepting Opening of $\vcom$]\label{def:accepting_opening_vcom}
For a sequence $\vcom=\{\com_{i}^{0},\com_{i}^{1}\}_{i=1}^{k}$ of commitments of the commitment scheme $\Com$, we say that $(\Vect{v}=(v_1,...,v_k),\Vect{r}=(r_1,...,r_k))$ is an accepting opening of $\vcom$ if the receiver of $\Com$ accepts the message $v_i$ with opening information $r_i$ in the decommit stage for all $i\in[k]$. 
\end{definition}


\begin{lemma}[Valid-Commitment $\epsilon$-Simulation Extractability]\label{lem:valid_com_extraction}
There exists a QPT algorithm $\SimExt$ such that for any noticeable $\epsilon(\secpar)$, any 
valid sequence of commitments $\vcom$ (in the sense of \Cref{def:valid_vcom}), and
any non-uniform QPT $C^*(\rho)$, 
\begin{equation}
\label{eq:valid_com_ext}
\left\{ \SimExt^{C^*(\rho)}(1^{\epsilon^{-1}}) \right\}_\secpar
\cind_\epsilon
\left\{\{(m^*, \ST_{C^*}):
\begin{array}{l}
\Vect{c}\gets \bit^k      
       \\
(\Vect{v},\Vect{r},\ST_{C^*}) \gets  C^*(\rho,\Vect{c})
\end{array}
\right\}_\secpar  
\end{equation}
where $m^*\defeq m_{\vcom}$ if $(\Vect{v},\Vect{r})$ is an accepting opening of $\vcom$ and otherwise $m^*\defeq \bot$.
\end{lemma}

==> sections/xiao_backup.tex <==
%!TEX root=../main.tex
The goal here is to show that the 4-round black-box ZK argument in \cite{TCC:HazVen18} is actually a 4-round black-box quantum $\epsilon$-ZK argument. 

The \cite{TCC:HazVen18} protocol makes use of the canonical extractable commitment (with the prover being the committer). I will first argue that this extractable commitment scheme, when instantiated with a  collapse-binding commitment as the basic $\Com$, will be extractable against a PQT committer (\Cref{sec:ext-PQT-com}). With this observation, I will present the construction together with an intuitive discussion of security proof in \Cref{sec:round_optimal_ezk}.

I must admit that I'm really a novice in quantum crypto. So don't hesitate to correct me if the following material is flawed in some fundamental way.

\section{Extractable Commitment Instantiated with Collapsing-Binding Com}
\label{sec:ext-PQT-com}
\begin{ProtocolBox}[
label={figure:ext-com},
% fontupper=\scriptsize,
float=!h,
]{Extractable Commitment Scheme}
\begingroup\fontsize{10pt}{0pt}\selectfont
The extractable commitment scheme, based on any commitment scheme $\Com$, works in the following way.\\
~\\
{\bf Input:}
\begin{itemize}[topsep=0.2em,itemsep=0.2em]
\item
both the sender (committer) $S$ and the receiver $R$ get security parameter $1^\SecPar$ as the common input.
\item
$S$ gets a string $\sigma \in \bits^{\ell(\SecPar)}$ as his private input, where $\ell(\cdot)$ is a polynomial 
\end{itemize}
~\\
{\bf Commitmment Phase:}
\begin{enumerate}[topsep=0.2em,itemsep=0.2em]
\item \label[Round]{item:extcom:com}
The sender (committer) $S$ commits using \Com to $k = \SecPar$ pairs of strings $\Set{(v^0_i, v^1_i)}_{i=1}^{k}$ where $(v^0_i ,v^1_i) = (\eta_i, \sigma \xor \eta_i)$ and $\eta_i$ are random strings in $\Set{0,1}^{|\sigma|}$ for $1 \le i \le k$.\footnotemark
\item \label[Round]{item:extcom:challenge}
Upon receiving a challenge $\Vect{c} = (c_1, \ldots, c_k)$ from the receiver $R$, $S$ opens the commitments to $(v^{c_1}_1, \ldots, v^{c_k}_k)$.
\item \label[Round]{item:extcom:open}
$R$ checks that the openings are valid.
\end{enumerate}
~\\
{\bf Decommitment Phase:}
\begin{itemize}[topsep=0.2em,itemsep=0.2em]
\item 
$S$ sends $\sigma$ and opens the commitments to all $k$ pairs of strings.
$R$ checks that all the openings are valid, and also that $\sigma = v^0_1 \xor v^1_1 = \cdots = v^0_k \xor v^1_k$.
\end{itemize}
\endgroup
\end{ProtocolBox}
\footnotetext{Actually, the scheme will be secure as long as we use \Com to commit $k = \omega(\log\SecPar)$ pairs of strings.}

Our starting point is the canonical extractable commitment shown in \Cref{figure:ext-com}. 
\begin{remark}[On the History]
This construction already existed implicitly in the implementation of concurrent zero-knowledge protocols in \cite{FOCS:PraRosSah02,TCC:Rosen04}. It was made explicit in \cite{TCC:MOSV06}, which also inherited the concurrent extractability from \cite{FOCS:PraRosSah02}. The standalone version was later formalized and used in several works, e.g., \cite{TCC:PasWee09,EC:GGJS12,EC:GarKiyPan17}. The version shown in \Cref{figure:ext-com} is taken from \cite{TCC:PasWee09}.
\end{remark}

\para{Recalling the Canonical Extractor.}
Given a PPT (potentially-malicious) sender $S^*$ that finishes the commitment phase with some non-negligible probability $\delta(\SecPar)$, the extractor $\Ext^{S^*}$ works in the following way. It first executes the protocol playing the role of the honest $R$. At the end of this execution, for each $i \in [k]$, $\Ext^{S^*}$ learns either $\eta_i$ or $\sigma \xor \eta_i$. It then rewinds $S$ to the beginning of \Cref{item:extcom:challenge}, samples a fresh $\Vect{c}'$, and finishes the execution. Since $\Vect{c} \ne \Vect{c}'$ except for negligible probability, it can be shown that, with probability $\approx \delta^2(\SecPar) - \negl(\SecPar)$, there is at least one $i \in [k]$ such that $\Ext^{S^*}$ learns {\bf both} $\eta_i$ and $\sigma \xor \eta_i$, which is sufficient for recovering the committed message $\sigma$. 

\para{Extraction from a Quantum $S^*$.} I have the following hope: if we instantiate the $\Com$ with a collapse-binding commitment in \Cref{figure:ext-com}, then the above extractor $\Ext$ should work even for a PQT $S^*$. My intuition is: the commitment in \Cref{figure:ext-com} is merely a parallel execution of $\Com$, and it is known that the collapse-binding property will be preserved under parallel repetition \cite{EC:Unruh16}. $\Ext$ does nothing more than a single rewinding. Therefore, following the techniques developed for quantum PoK \cite{EC:Unruh12,EC:Unruh16}, we should be able to prove that $\Ext$ can finish the rewinding successfully with a PQT $S^*$, thus extracting the committed value $\sigma$. \red{(Let me know if I'm wrong.)}





\section{4-Round Black-Box $\epsilon$-ZK Arguments}
\label{sec:round_optimal_ezk}
If what I said in \Cref{sec:ext-PQT-com} is correct, then I think we will have a black-box $\epsilon$-ZK argument in 4 rounds, assuming either QLWE or injective OWF (quantumly-oneway). The construction (shown in \Cref{figure:round_optimal_ZK}) is identical to the protocol in \cite{TCC:HazVen18}, except the we instantiated the commitment schemes differently. Formally, we need the following building blocks:
\begin{itemize}
\item
A non-interactive commitment scheme $\SBCom$ that is (quantumly) computationally-hiding and statistically-binding. Such a scheme can be constructed from QLWE \cite{lombardi2019note}, or injective OWF (quantumly-oneway) in general. 
\item
The extractable commitment as in \Cref{figure:ext-com}, where $\Com$ is a 2-round computationally-hiding, collapse-binding commitment.
\item
The $\Sigma$-protocol $\Prot_\textsc{ham}$ for Hamiltonicity, satisfying the same requirements as in your paper \cite[Definition 6.2]{chia2020black}.
\end{itemize}




\begin{ProtocolBox}[
label={figure:round_optimal_ZK},
% fontupper=\scriptsize,
float=!h,
]{4-Round Black-Box $\epsilon$-ZK Arguments}
\begingroup\fontsize{10pt}{0pt}\selectfont

\begin{enumerate}[topsep=0.5em,itemsep=0.5em]
\item \label[Round]{item:ezk:round:1}
$V$ picks $n$ challenges $\Set{e_1, \ldots, e_n}$ for the parallel invocations of protocol $\Prot_\textsc{ham}$, and commits to them separately using $\SBCom$.
\item \label[Round]{item:ezk:round:2}
$P$ generates $n$ first-messages $(a_1, \ldots, a_n)$, corresponding to $n$ parallel repetition of $\Prot_\textsc{ham}$. Here, each $a_i$ is a commitment to the (permuted) graph. We require that $P$ uses the \Cref{item:extcom:com} of the $\ExtCom$ (\Cref{figure:ext-com}) as the commitment scheme.
\item \label[Round]{item:ezk:round:3}
$V$ sends to $P$ two types of challenges:
\begin{itemize}[topsep=0.5em,itemsep=0.5em]
\item 
$\Prot_\textsc{ham}$ {\bf Challenges:}
It samples a size-$t$ (say, $t$ is a constant fraction of $n$) random subset $T \subset [n]$, and decommit to $\Set{e_i}_{i \in T}$. Looking ahead, this is the verifier's challenges to the $\Prot_\textsc{ham}$ protocol. 
\item 
$\ExtCom$ {\bf Challenges:}
For the remaining $n -t$ ``slots'', $V$ does not execute $\Prot_\textsc{ham}$. Instead, it samples $n-t$ random bits $\Set{c_1, \ldots, c_{n-t}}$ and send them to $P$. Looking ahead, these bits play the role of the \Cref{item:extcom:challenge} message of the $\ExtCom$ (\Cref{figure:ext-com}).
\end{itemize}
\item \label[Round]{item:ezk:round:4}
$P$ responds in the following way:
\begin{itemize}
\item
For $\Set{e_i}_{i \in T}$, $P$ responds as the $\Prot_\textsc{ham}$ prover.
\item
For $\Set{c_1, \ldots, c_{n-t}}$, $P$ responds as the $\ExtCom$ committer. That is, $P$ sends the 
\end{itemize}
\end{enumerate}
{\bf Verifier's decision:} $V$ does the verification in the natural way: it accepts iff both types of challenges are answered convincingly.
\endgroup
\end{ProtocolBox}

\subsection{The Intuition for the Security}
Completeness is obvious.

\para{The $\epsilon$-ZK Property.} The $\epsilon$-ZK property can be proved in a similar manner as in your paper \cite{chia2020black}. That is, the $\Sim_\textsf{na}$ will invoke your extraction lemma on the $\SBCom$ in \Cref{item:ezk:round:1} of \Cref{figure:round_optimal_ZK}. Once the committed $\Set{e_1, \ldots, e_n}$ are extracted, the simulation can be done easily. \red{(Let me known if I'm wrong.)}

\begin{remark}
Proving the (classical) ZK property in their original paper \cite{TCC:HazVen18} is a super-hard task. It involves a complicate combinatorial analysis, which indeed constitutes their main technical contribution.
\end{remark} 

\para{The Soundness.} Let me first explain how the authors of \cite{TCC:HazVen18} proved (classical) soundness. At the high-level, they reduced the soundness to the computationally-hiding property of the $\SBCom$ in \Cref{item:ezk:round:1}. Observe that in \Cref{item:ezk:round:3} of \Cref{figure:round_optimal_ZK}, $V$ sends two types of challenges. In particular, the $\Prot_\textsc{ham}$-challenges ensure that the $P^*$ prepares (most of) the $\Set{a_1, \ldots, a_n}$ messages following the requirement of $\Prot_\textsc{ham}$. Thus, if $P^*$ wants to cheat, the only way is to predict the $\Set{e_1, \ldots, e_n}$ values committed in $\SBCom$.

Also, note that the $\Set{a_i}_{i\in [n]}$ are commits using the $\ExtCom$ (as in \Cref{figure:ext-com}) (where the \Cref{item:extcom:challenge} and \Cref{item:extcom:open} of the commitment phase appear as the $\ExtCom$-challenge and response in \Cref{figure:round_optimal_ZK}). Therefore, we can invoke the $\ExtCom$ extractor on $P^*$ to extract the value committed in $\Set{a_1, \ldots, a_n}$.\footnote{Note that we can only extract values form some of $\Set{a_i}$, but not all. Because some of them (with indices in the set $T$) were used for $\Prot_\textsc{ham}$ check. But this is sufficient for proving soundness.} We can read out $P^*$'s prediction of $\Set{e_1, \ldots, e_n}$ from these extracted values, thanks to the ``bad challenge searchability'' of $\Prot_\textsc{ham}$. This contradicts the computational-hiding of $\SBCom$.

It can be seen that the core of the above soundness proof is to ensure that we can rewind $P^*$ to extract the values committed in $\Set{a_1, \ldots, a_n}$. Now, consider the $\ExtCom$ in \Cref{sec:ext-PQT-com}. If its extractor $\Ext$ indeed works for PQT committers, then the above classical soundness proof for \Cref{figure:round_optimal_ZK} will extend naturally to rule out a PQT cheating prover $P^*$. 

\para{The Argument of Knowledge Property.} \red{I just realized that this protocol won't be an arguemnt of knowledge. Becuase the value extracted from $\ExtCom_i$ for $i \notin T$ can't tell us anything about the witness (e.g., it could simply be a randomly permuted of the graph $G$).

To get a ZKAoK, we may need to extend the extraction lemma to the protocol from \cite[Fig.\ 3]{TCC:KhuOstSri18}. That protocol relies on a clever use of randomized encoding. Also, the verifier there uses a special commitment. It is interesting to see if we can extend the extraction lemma to that special commitment.
}
%I feel that the above protocol is also an argument of knowledge, though the authors of \cite{TCC:HazVen18} did not claim that. My intuition is: in the soundness proof, the rewinding procedure will not only extract for the $\ExtCom$-challenges; it also extracts for the $\Prot_\textsc{ham}$-challenges. That is, there exist an $i\in [n]$ for which the extractor will see both the committed graph and its Hamiltonian circle (responses to both the $b=0$ and $b=1$ challenges of the underlying $\Prot_\textsc{ham}$ protocol). This should be sufficient for extracting the witness.  

\section{Extending the Extraction-Simulation Lemma to ExtCom}
I think this is possible. We need to make the extractor depend on the ExtCom challenges. Concretely, in the $\Ext(1^\SecPar, \mathsf{pp}, \mathsf{com}, \Adv_{\mathsf{open}, \SecPar}, \rho_{\mathsf{st}})$ from \cite{chia2020black}, we make the following changes:
\begin{itemize}
    \item take an additional parameter $\mathsf{ch} = (c_1, \ldots, c_k)$. This is the receiver's challenge vector in the commitment phase of $\ExtCom$.
    \item Make the $\Pi_{\mathsf{open}}$ depend on $\mathsf{ch}$. That is, open only the positions specified by $\mathsf{ch}$. Notice that this also affects the construction of the amplifier, which depends on $\mathsf{open}$.
    \item
    Execute the extractor $\Ext$ as in \cite{chia2020black} up to step 6. Now the $\rho_{\Ext}$ should be negligible close to $\rho_{\mathsf{st}}$, if we are run the amplifier to super-polynomial time.  
    \item
    Now, run $\Ext(1^\SecPar, \mathsf{pp}, \mathsf{com}, \Adv_{\mathsf{open}, \SecPar}, \rho_{\Ext}, \mathsf{ch}')$, where $\mathsf{ch}'$ is a freshly-sampled $(c_1', \ldots, c_k')$ (of course, the $\Pi_{\mathsf{open}}$ is modified accordingly).
\end{itemize}
The above procedure should make sure that we learn responses for both $\mathsf{ch}$ and $\mathsf{ch}'$, which is enough to extracted the committed value. And the final $\rho_\Ext$ (form the second run of $\Ext$) should be still negligibly close to $\rho_{\mathsf{st}}$.
